HUWSOD: Holistic Self-training for Unified Weakly Supervised Object Detection

Weakly supervised object detection~(WSOD) trains object detectors using only image-level annotations. Most existing methods rely on offline object proposals to generate candidate regions and suffer from unstable optimization that can converge to poor local optima. We present HUWSOD, a unified, high-capacity WSOD framework with holistic self-training. The framework is self-contained and requires neither external proposal modules nor additional supervision. First, a self-supervised proposal generator and an autoencoder proposal generator, equipped with a multi-rate resampling pyramid, hypothesize object locations. They replace traditional proposals and enable end-to-end training and inference. Second, holistic self-training combines step-wise entropy minimization with consistency-constraint regularization to progressively refine detection scores and box coordinates while enforcing agreement between predictions from stochastic augmentations of the same image. Extensive experiments on PASCAL VOC and MS COCO show that HUWSOD is competitive with state-of-the-art WSOD methods without offline proposals or additional data. With class-agnostic ground-truth bounding boxes, its upper-bound performance approaches that of Faster R-CNN, demonstrating the potential to attain fully supervised accuracy. We further find that randomly initialized boxes, although substantially different from carefully designed offline proposals, can serve as effective object candidates for WSOD training.

==> main/head.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}




\usepackage{subcaption}
%\captionsetup{compatibility=false}
\usepackage{caption}
\usepackage{newfloat}
\usepackage{listings}
\usepackage{xspace}

\usepackage{graphbox}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{wrapfig}
\usepackage{tikz}
\usepackage{float}

\usepackage[export]{adjustbox}
\usepackage{booktabs}
\usepackage{stackengine}
\usepackage{tablefootnote}
\usepackage{threeparttable}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{dsfont}

\usepackage{color}
\usepackage{colortbl}
\usepackage[inline, shortlabels]{enumitem}
\usepackage{ifthen}
\usepackage{ragged2e}
\usepackage[normalem]{ulem}

\newcommand{\hfilll}{\hspace{0pt plus 1filll}}

\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

%\makeatletter
%\@namedef{ver@everyshi.sty}{}
%\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmin}{arg\,min} % thin space, limits underneath in displays
%\DeclareMathOperator*{\argmin}{argmin} % no space, limits underneath in displays
%\DeclareMathOperator{\argmin}{arg\,min} % thin space, limits on side in displays
%\DeclareMathOperator{\argmin}{argmin} % no space, limits on side in displays

% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\captionsetup[table]{position=top}

\setlength{\textfloatsep}{10pt}
\setlength{\floatsep}{10pt}
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{0pt}

\setlength{\dbltextfloatsep}{10pt}
\setlength{\dblfloatsep}{10pt}

\setlength{\tabcolsep}{3pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage[backref=page,colorlinks]{hyperref}
%\usepackage[colorlinks]{hyperref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\def\OurMethod{HUWSOD\xspace}
\def\OurMethodx{HUWSOD$^*$\xspace}
\def\placeholder{{\color{red}xxxx xxxx}}
\makeatother



%% IJCV
\usepackage[numbers]{natbib}
\usepackage[colorlinks,linkcolor=red,anchorcolor=blue,citecolor=blue,CJKbookmarks=True]{hyperref}




==> main/table_coco_sota_map_net.tex <==
\begin{table*}[t]
    \centering
    %\vspace{-15pt}
    \caption{Result comparison with the state-of-the-art methods on COCO val set.}
%    \vspace{-10pt}
    %\footnotesize
    \begin{center}
        \begin{adjustbox}{max width=0.7\linewidth}
            \centering
            %\vspace{-5.0pt}
            \begin{tabular}{l|c|ccc|ccc}
                \hline
                \multirow{2}{*}{Method} & \multirow{2}{*}{Bakcbone} & \multicolumn{3}{c|}{\scriptsize{Avg. Precision, IoU:}} & \multicolumn{3}{c}{\scriptsize{Avg. Precision, Area:}}\\
                % & \multicolumn{3}{c|}{\scriptsize{Avg. Recall, \#Dets:}} & \multicolumn{3}{c}{\scriptsize{Avg. Recall, Area:}}\\
                & & 0.5:0.95 & 0.5 & 0.75 & S & M & L \\
                %& 1 & 10 & 100 & S & M & L\\
                
                %==============================================================================================================
                \hline
                
                % wsddn_vgg16_coco_2019-07-03_01-19-17
%                WSDDN$^*$                                                          &VGG16&10.2&20.4&08.8&02.2&11.0&18.9&13.0&24.8&26.9&05.7&29.6&50.2\\
%                WSDDN$^*$                                                          &VGG16&10.2&20.4&08.8&02.2&11.0&18.9\\
                
                % wsddn_vgg_cnn_m_coco_2019-07-31_02-58-46
%                WSDDN$^*$                                                          &VGG-M&08.8&17.1&07.9&01.3&08.4&15.9&11.7&21.9&23.6&04.1&23.6&46.2\\
%                WSDDN$^*$                                                          &VGG-M&08.8&17.1&07.9&01.3&08.4&15.9\\
                
                % wsddn_vgg_cnn_f_coco_2019-07-30_17-30-43
%                WSDDN$^*$                                                          &VGG-F&08.6&16.5&07.8&01.6&08.8&15.3&11.4&21.7&23.3&04.0&23.7&45.7\\
%                WSDDN$^*$                                                          &VGG-F&08.6&16.5&07.8&01.6&08.8&15.3\\
                
                % csc_vgg16_coco_2019-07-05_01-54-02
%                CSC C5                                                             &VGG16&10.2&20.3&08.9&02.3&10.9&18.5&13.0&24.8&26.7&05.2&28.6&50.2\\
%                CSC C5                                                             &VGG16&10.2&20.3&08.9&02.3&10.9&18.5\\
                
                % paper
%                WSDDN \hfilll\cite{Bilen2016}                                      &VGG16&9.5&19.2&8.2&2.1&10.4&17.2&12.2&23.6&25.3&6.3&25.7&48.2\\
                WSDDN \hfilll\cite{Bilen2016}                                      &VGG16&9.5&19.2&8.2&2.1&10.4&17.2\\
                
                % paper
%                ContextLocNet\hfilll\cite{Kantorov2016}                            &VGG16&11.1&22.1&10.7&{2.9}&12.4&19.2&{12.2}&{24.5}&24.3&{6.5}&28.7&49.3\\
                ContextLocNet\hfilll\cite{Kantorov2016}                            &VGG16&11.1&22.1&10.7&{2.9}&12.4&19.2\\
                
                % paper
%                CSC C5\hfilll\cite{Shen_2019_TIP}                                  &VGG16&{12.9}&{23.8}&{13.2}&{2.9}&{12.5}&{20.3}&{12.2}&23.9&{25.7}&6.1&{29.7}&{49.7}\\
%                CSC C5\hfilll\cite{Shen_2019_TIP}                                  &VGG16&{12.9}&{23.8}&{13.2}&{2.9}&{12.5}&{20.3}\\
                
%                Diba \etal\hfilll\cite{Diba2017a}        &VGG16(14train/14test)&--&12.8&--&--&--&--\\
                
%                SD-LocNet\hfilll\cite{Zhang2019b}        &VGG16(14train/14val)&9.7&21.6&--&--&--&--\\
                
                ML-LocNet\hfilll\cite{Zhang2018g}        &VGG-S&--&16.2&--&--&--&--\\
                
                WSOD$^2$\hfilll\cite{Zeng2019}          &VGG16&10.8&22.7&--&--&--&--\\
                
%                PCL\hfilll\cite{Tang2018b}&VGG-M(14train/14val)&7.3&16.6&--&--&--&--\\
                PCL\hfilll\cite{Tang2018b}&VGG16&8.5&19.4&--&--&--&--\\
%                PCL Fast RCNN\hfilll\cite{Tang2018b}&VGG16(14train/14val)&9.2&19.6&--&--&--&--\\
                
                C-MIDN\hfilll\cite{CMIDN}&VGG16&9.6&21.4&--&--&--&--\\
                
                PG-PS\hfilll\cite{Cheng2020}&VGG16&--&20.7&--&--&--&--\\
                
%                PML-LocNet-S\hfilll\cite{Zhang2020a}&VGG16(14train/14val)&--&21.6&--&--&--&--\\
%                PML-LocNet-L\hfilll\cite{Zhang2020a}&VGG16(14train/14val)&--&20.9&--&--&--&--\\
                
                %==============================================================================================================
                %\hline
                
                %\multirow{4}{*}{WSDDN}\hfilll\multirow{4}{*}{\cite{Bilen2016}}&VGG16&9.5&19.2&8.2&2.1&10.4&17.2\\
                %&12.2&23.6&25.3&6.3&25.7&48.2\\
                %&ResNet18-WS&11.3&22.0&10.0&2.7&11.9&21.4\\
                %&ResNet50-WS&\\%TODO
                %&ResNet101-WS&\\%TODO
                
                %==============================================================================================================
                %\hline
                
                %\multirow{4}{*}{ContextNet}\hfilll\multirow{4}{*}{\cite{Kantorov2016}}&VGG16&11.1&22.1&10.7&{2.9}&12.4&19.2\\
                %&{12.2}&{24.5}&24.3&{6.5}&28.7&49.3\\
                %&ResNet18-WS&15.0&25.9&13.8&4.2&15.1&24.4\\%TODO
                %&ResNet50-WS&\\%TODO
                %&ResNet101-WS&\\%TODO
                
                %==============================================================================================================
%                \hline
                
                \multirow{1}{*}{Ren \etal}\hfilll\multirow{1}{*}{\cite{Ren2020}}
%                &VGG16(14train/14val)&11.4&24.3&9.4&3.6&12.2&17.6\\
%                &R50-C4(14train/14val)&12.6&26.1&10.8&3.7&13.3&19.9\\
%                &R101-C4(14train/14val)&13.0&26.3&11.4&3.5&13.7&20.4\\
                &VGG16&12.4&25.8&10.5&3.9&13.8&19.9\\
%                &VGG16(14train/Test-Dev)&12.1&24.8&10.2&4.1&13.0&18.3\\
                
                %==============================================================================================================
                \hline
                UWSOD&VGG16&\textbf{16.1}&\textbf{30.9}&\textbf{14.8}&\textbf{5.0}&\textbf{17.1}&\textbf{27.5}\\
                
                
                %==============================================================================================================
                \hline
                \multicolumn{7}{c}{FSOD}\\
                \hline
                
                Fast RCNN\hfilll\cite{FASTRCNN}&VGG16&18.9&38.6&--&--&--&--\\
                Faster RCNN\hfilll\cite{FASTERRCNN}&VGG16&21.2&41.5&--&--&--&--\\
                
                %==============================================================================================================
                \hline
            \end{tabular}
            %\vspace{-5.0pt}
        \end{adjustbox}
    \end{center}
%    \vspace{-20pt}
    \label{table_coco_sota_map_sm}
\end{table*}


==> main/table_voc2007_abl_aeopg_crst.tex <==

\begin{table*}[t]
    
    
    \begin{minipage}[t]{.5\linewidth}
        
        %\begin{table}[t]
        %\vspace{-20pt}
        \caption{
            Ablation study of AEOPG on the VOC 2007 test set in terms of mAP~(\%) and CorLoc~(\%).
        }
        %\vspace{-5pt}
        %\footnotesize
        \begin{center}
            \begin{adjustbox}{max width=1.0\linewidth}
                \begin{tabular}{c|c|c|c|c|c|c|c}
                    \toprule
                    
                    &$\mathcal{L}_\mathrm{Encoder}$&$\mathcal{L}_\mathrm{Decoder}$&$E$&$q$&$D$&CorLoc&\emph{m}AP\\
                    
                    %==============================================================================================================
                    \midrule
                    
                    baseline&--&--&--&--&--&
                    63.0&44.0\\
                    
                    \midrule
                    
                    a&\checkmark&--&$(C, 32, 2)$&$1$&-&
                    &\\
                    
                    b&&\checkmark&$(C, 32, 2)$&$1$&$(32, C, 2)$&
                    &\\
                    
                    c&\checkmark&\checkmark&$(C, 32, 2)$&$1$&$(32, C, 2)$&68.0
                    &50.2\\
                    
                    
                    \midrule
                    
                    d&\checkmark&\checkmark&$(C, 32, 2)$&$2$&$(32, C, 2)$&
                    &\\
                    
                    e&\checkmark&\checkmark&$(C, 32, 2)$&$3$&$(32, C, 2)$&
                    &\\
                    
                    f&\checkmark&\checkmark&$(C, 32, 2)$&$4$&$(32, C, 2)$&
                    &\\
                    
                    \midrule
                    
                    g&\checkmark&\checkmark&$(C, 16, 2)$&$1$&$(16, C, 2)$&
                    &\\
                    
                    h&\checkmark&\checkmark&$(C, 32, 4)$&$1$&$(32, C, 4)$&
                    &\\
                    
                    i&\checkmark&\checkmark&$(C, 8, 4)$&$1$&$(8, C, 4)$&
                    &\\
                    
                    %==============================================================================================================
                    \bottomrule
                \end{tabular}
            \end{adjustbox}
        \end{center}
        %    \vspace{-20pt}
        \label{table_voc2007_abl_aeopg}
        %\end{table}
        
        
    \end{minipage}
    \hspace{2pt}
    \begin{minipage}[t]{.5\linewidth}
        
        
        %\begin{table}[t]
        %\vspace{-20pt}
        \caption{
            Ablation study of CCR on the VOC 2007 test set in terms of mAP~(\%) and CorLoc~(\%).
        }
        %\vspace{-5pt}
        %\footnotesize
        \begin{center}
            \begin{adjustbox}{max width=1.0\linewidth}
                \begin{tabular}{c|c|c|c|c|c|c|c|c}
                    \toprule
                    
                    &$| \mathcal{T} |$&color jitter&gray scale&blur&cutout&$\beta$&CorLoc&\emph{m}AP\\
                    
                    %==============================================================================================================
                    \midrule
                    
                    a&--&--&--&--&--&--&
                    &\\
                    
                    \midrule
                    
                    b&1&\checkmark&--&--&--&--&
                    &\\
                    
                    c&1&\checkmark&\checkmark&--&--&--&
                    &\\
                    
                    d&1&\checkmark&\checkmark&\checkmark&--&--&
                    &\\
                    
                    e&1&\checkmark&\checkmark&\checkmark&\checkmark&--&67.9
                    &49.7\\
                    
                    \midrule
                    
                    f&2&\checkmark&\checkmark&\checkmark&\checkmark&--&
                    &\\
                    
                    g&3&\checkmark&\checkmark&\checkmark&\checkmark&--&
                    &\\
                    
                    h&4&\checkmark&\checkmark&\checkmark&\checkmark&--&
                    &\\
                    
                    \midrule
                    
                    i&1&\checkmark&\checkmark&\checkmark&\checkmark&0.999&
                    &\\
                    
                    j&1&\checkmark&\checkmark&\checkmark&\checkmark&0.9999&
                    &\\
                    
                    k&1&\checkmark&\checkmark&\checkmark&\checkmark&0.99999&
                    &\\
                    
                    l&1&\checkmark&\checkmark&\checkmark&\checkmark&0.99999&
                    &\\
                    
                    %==============================================================================================================
                    \bottomrule
                \end{tabular}
            \end{adjustbox}
        \end{center}
        %    \vspace{-20pt}
        \label{table_voc2007_abl_crst}
        %\end{table}
        
        
    \end{minipage}
    
    %\vspace{-9pt}
\end{table*}

==> main/table_voc2007_sota_CorLoc.tex <==
\begin{table*}[t]
    \caption{
        %Comparison with the state-of-the-art methods on PASCAL VOC 2007 in terms of CorLoc (\%) on train set.
        Comparison with the state-of-the-art methods on VOC 2007 in terms of CorLoc on train set.
    }
    \vspace{-10pt}
    \footnotesize
    \begin{center}
        \begin{adjustbox}{max width=1.0\linewidth}
            \begin{tabular}{l|cccccccccccccccccccc|c}
                \hline
                
                Method&aero&bicy&bird&boa&bot&bus&car&cat&cha&cow&dtab&dog&hors&mbik&pers&plnt&she&sofa&trai&tv&Av.\\
                
                \hline
                \multicolumn{22}{c}{Object Mining}\\
                %==============================================================================================================
                \hline
                
                %Siva \etal\hfilll\cite{siva2012defence}&&45.8&21.8&30.9&20.4&5.3&37.6&40.8&51.6&7.0&29.8&27.5&41.3&41.8&47.3&24.1&12.2&28.1&32.8&48.7&9.4&30.2\\
                
                %Shi \etal\hfilll\cite{Shi2017}&&67.3&54.4&34.3&17.8&1.3&46.6&60.7&68.9&2.5&32.4&16.2&58.9&51.5&64.6&18.2&3.1&20.9&34.7&63.4&5.9&36.2\\
                
                %LCL-pLSA\hfilll\cite{Wang2014}&80.1&63.9&51.5&14.9&21.0&55.7&74.2&43.5&26.2&53.4&16.3&56.7&58.3&69.5&14.1&38.3&58.8&47.2&49.1&60.9&48.5\\
                
                %Bilen \etal\hfilll\cite{Bilen2015}&66.4&59.3&42.7&20.4&21.3&63.4&74.3&59.6&21.1&58.2&14.0&38.5&49.5&60.0&19.8&39.2&41.7&30.1&50.2&44.1&43.7\\
                
                %Multi-Fold MIL\hfilll\cite{Cinbis2015}&65.3&55.0&52.4&48.3&18.2&66.4&77.8&35.6&26.5&67.0&46.9&48.4&70.5&69.1&35.2&35.2&69.6&43.4&64.6&43.7&52.0\\
                
                %Rochan\hfilll\cite{Rochan2015}&78.6&63.4&66.4&56.4&19.7&82.3&74.8&69.1&22.5&72.3&31&63.0&74.9&78.4&48.6&29.4&64.6&36.2&75.9&69.5&58.8\\
                
                %RMI-SVM\hfilll\cite{Wang2015}&37.7&58.8&39.0&4.7&4.0&48.4&70.0&63.7&9.0&54.2&33.3&37.4&61.6&57.6&30.1&31.7&32.4&52.8&49.0&27.8&40.2\\
                
                %STL\hfilll\cite{Bazzani2016}&79.0&55.6&48.8&47.0&17.2&64.5&63.8&84.6&19.5&68.8&49.5&61.3&65.2&74.3&35.1&26.5&58.3&56.8&78.9&33.2&54.4\\
                
                %Teh\hfilll\cite{Teh2016}&84.0&64.6&70.0&62.4&25.8&80.7&73.9&71.5&35.7&81.6&46.5&71.3&79.1&78.8&56.7&34.3&69.8&56.7&77.0&72.7&64.6\\
                
                %WSDDN\hfilll\cite{Bilen2016}&68.5&67.5&56.7&34.3&32.8&69.9&75.0&45.7&17.1&68.1&30.5&40.6&67.2&82.9&28.8&43.7&71.9&62.0&62.8&58.2&54.2\\
                %WSDDN\hfilll\cite{Bilen2016}&65.1&63.4&59.7&45.9&38.5&69.4&77.0&50.7&30.1&68.8&34.0&37.3&61.0&82.9&25.1&42.9&79.2&59.4&68.2&64.1&56.1\\
                WSDDN\hfilll\cite{Bilen2016}&65.1&58.8&58.5&33.1&39.8&68.3&60.2&59.6&34.8&64.5&30.5&43.0&56.8&82.4&25.5&41.6&61.5&55.9&65.9&63.7&53.5\\
                
                ContextLocNet\hfilll\cite{Kantorov2016}&83.3&68.6&54.7&23.4&18.3&73.6&74.1&54.1&8.6&65.1&47.1&59.5&67.0&83.5&35.3&39.9&67.0&49.7&63.5&65.2&55.1\\
                
                OM + MIL\hfilll\cite{Li2016}&64.3&54.3&42.7&22.7&34.4&58.1&74.3&36.2&24.3&50.4&11.0&29.2&50.5&66.1&11.3&42.9&39.6&18.3&54.0&39.8&41.2\\
                
                %OPG\hfilll\cite{Shen_2018_TNNLS}&44.5&33.7&36.1&16.6&7.0&38.2&42.0&57.6&8.5&30.5&29.0&43.2&55.4&56.0&27.6&18.8&36.5&38.9&49.4&14.5&34.2\\
                %OPG\hfilll\cite{Shen_2018_TNNLS}&57.1&43.2&53.9&23.8&12.3&47.9&48.8&69.1&16.6&47.5&39.0&61.3&54.7&60.8&32.1&22.0&49.0&44.1&59.4&27.7&43.5\\
                
                WCCN\hfilll\cite{Diba2017}&83.9&72.8&64.5&44.1&40.1&65.7&82.5&58.9&33.7&72.5&25.6&53.7&67.4&77.4&26.8&49.1&68.1&27.9&64.5&55.7&56.7\\
                
                Jie \etal'17\hfilll\cite{Jie2017}&72.7&55.3&53.0&27.8&35.2&68.6&81.9&60.7&11.6&71.6&29.7&54.3&64.3&88.2&22.2&53.7&72.2&52.6&68.9&75.5&56.1\\
                
                SP-VGGNet\hfilll\cite{Zhu2017}&85.3&64.2&67.0&42.0&16.4&71.0&64.7&88.7&20.7&63.8&58.0&84.1&84.7&80.0&60.0&29.4&56.3&68.1&77.4&30.5&60.6\\
                
                TST\hfilll\cite{Shi2017a}&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&59.5\\
                
                SGWSOD\hfilll\cite{Lai2017a}&74.4&74.1&54.2&44.2&38.1&78.0&82.9&62.3&21.6&71.6&31.0&59.1&74.2&85.7&43.6&49.8&72.9&62.5&65.5&69.9&60.8\\
                %SGWSOD\hfilll\cite{Lai2017a}&VGG-M-1024&74.8&72.0&47.0&40.3&37.7&74.7&84.4&63.8&25.8&66.7&38.5&48.0&68.3&83.7&40.7&52.2&74.0&59.8&66.7&72.7&59.6\\
                %SGWSOD\hfilll\cite{Lai2017a}&71.0&76.5&54.9&49.7&54.1&78.0&87.4&68.8&32.4&75.2&29.5&58.0&67.3&84.5&41.5&49.0&78.1&60.3&62.8&78.9&62.9\\
                
                TS$^2$C\hfilll\cite{Wei2018TS2C}&84.2&74.1&61.3&52.1&32.1&76.7&82.9&66.6&42.3&70.6&39.5&57.0&61.2&88.4&9.3&54.6&72.2&60.0&65.0&70.3&61.0\\
                
                %CSC C5\hfilll\cite{Shen_2019_TIP}&77.3&75.7&63.9&33.7&41.0&75.8&77.3&72.4&20.9&73.8&35.0&52.7&77.0&83.7&46.2&43.3&69.8&64.6&80.5&43.4&60.4\\
                %CSC C5\hfilll\cite{Shen_2019_TIP}&68.9&75.7&68.5&32.6&43.4&75.3&80.2&75.7&13.3&70.2&15.5&63.0&72.8&80.8&57.7&48.2&71.9&59.0&76.3&62.9&60.6\\
                %CSC C5\hfilll\cite{Shen_2019_TIP}&76.1&75.3&61.8&42.0&54.1&74.7&78.8&67.4&32.8&73.1&46.5&59.9&37.6&78.0&56.0&42.5&71.9&67.3&82.4&65.6&62.2\\
                
                %WS-JDS\hfilll\cite{Shen_2019_CVPR}&82.9&74.0&73.4&47.1&60.9&80.4&77.5&78.8&18.6&70.0&56.7&67.0&64.5&84.0&47.0&50.1&71.9&57.6&83.3&43.5&64.5\\
                
                %==============================================================================================================
                %\hline
                %\multirow{4}{*}{WSDDN}\hfilll\multirow{4}{*}{\cite{Bilen2016}}&65.1&58.8&58.5&33.1&39.8&68.3&60.2&59.6&34.8&64.5&30.5&43.0&56.8&82.4&25.5&41.6&61.5&55.9&65.9&63.7&53.5\\
                %&ResNet18-WS &75.0&63.7&65.0&37.0&60.4&80.4&81.1&70.5&21.8&60.8&65.9&44.3&74.8&85.0&37.5&56.3&68.7&63.9&74.0&75.0&63.1\\
                %&ResNet50-WS &74.1&68.9&69.4&39.5&64.0&79.3&84.3&66.2&42.4&73.9&38.1&52.7&69.7&83.3&27.2&54.8&68.7&57.6&81.8&75.7&63.6\\
                %&ResNet101-WS&72.3&63.7&67.7&49.3&61.8&77.3&85.1&63.8&36.1&68.1&45.3&52.2&71.2&87.5&27.9&58.6&66.6&66.6&76.3&81.2&64.0\\
                
                %==============================================================================================================
                %\hline
                %\multirow{4}{*}{ContextLocNet}\hfilll\multirow{4}{*}{\cite{Kantorov2016}}&83.3&68.6&54.7&23.4&18.3&73.6&74.1&54.1&8.6&65.1&47.1&59.5&67.0&83.5&35.3&39.9&67.0&49.7&63.5&65.2&55.1\\
                %&ResNet18-WS &82.1&62.9&66.6&44.4&53.2&80.4&84.5&82.2&22.7&60.8&60.8&68.4&76.2&84.1&29.5&55.6&64.5&68.4&76.3&70.3&64.7\\
                %&ResNet50-WS &74.0&77.8&63.5&43.6&58.0&81.6&79.6&68.0&25.2&79.5&59.5&60.0&61.3&81.1&54.5&47.3&82.5&62.3&75.7&65.9&65.1\\ %TODO
                %&ResNet101-WS&81.7&78.7&65.3&56.0&56.2&77.5&82.2&73.0&32.1&81.9&36.9&62.8&67.6&84.0&55.2&57.1&70.8&64.4&731.&57.0&65.7\\ %TODO
                
                %==============================================================================================================
                \hline
                \multicolumn{22}{c}{Object Mining + Instance Refinement}\\
                
                %==============================================================================================================
                \hline
                
                %OICR\hfilll\cite{Tang2017}&81.7&72.9&56.5&31.4&36.3&75.6&81.6&57.0&7.3&74.7&47.1&46.0&78.2&88.8&12.2&46.2&66.0&56.7&65.8&64.9&57.3\\
                OICR\hfilll\cite{Tang2017}&81.7&80.4&48.7&49.5&32.8&81.7&85.4&40.1&40.6&79.5&35.7&33.7&60.5&88.8&21.8&57.9&76.3&59.9&75.3&81.4&60.6\\
                
                %K-EM\hfilll\cite{Yan2017}&79.8&77.8&66.7&50.3&57.0&80.1&89.9&71.5&29.9&75.9&30.5&58.9&73.2&90.2&25.4&51.8&80.2&60.3&72.4&78.9&65.0\\
                
                MELM\hfilll\cite{Wan}&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&61.4\\
                
                ZLDN\hfilll\cite{Zhang2018b}&74.0&77.8&65.2&37.0&46.7&75.8&83.7&58.8&17.5&73.1&49.0&51.3&76.7&87.4&30.6&47.8&75.0&62.5&64.8&68.8&61.2\\
                
                %GAL-fWSD300\hfilll\cite{Shen_2018_CVPR}&76.5&76.1&64.2&48.1&52.5&80.7&86.1&73.9&30.8&78.7&62.0&71.5&46.7&86.1&60.7&47.8&82.3&74.7&83.1&79.3&68.1\\
                %GAL-fWSD512\hfilll\cite{Shen_2018_CVPR}&78.6&81.9&63.6&40.3&48.8&80.7&85.3&76.3&30.3&78.0&54.5&65.3&48.4&86.5&56.3&46.9&76.0&68.1&83.9&73.1&66.1\\
                
                %ML-LocNet\hfilll\cite{Zhang2018g}&VGG-S&76.9&78.2&65.8&39.8&45.9&78.0&85.1&57.0&16.9&70.9&68.5&56.5&77.0&90.6&47.4&52.2&65.6&60.7&75.5&65.2&63.7\\
                ML-LocNet\hfilll\cite{Zhang2018g}&78.0&78.5&66.2&43.2&51.5&76.5&86.8&65.7&34.9&69.5&59.7&55.1&79.5&88.1&40.3&58.3&71.5&64.0&77.0&61.6&65.3\\
                ML-LocNet\hfilll\cite{Zhang2018g}&78.6&82.3&68.2&42.0&53.3&78.5&88.5&70.3&36.4&70.2&60.5&58.0&80.5&88.2&38.8&59.2&75.0&69.0&78.2&64.5&67.0\\
                
                WSRPN\hfilll\cite{Tang}&77.5&81.2&55.3&19.7&44.3&80.2&86.6&69.5&10.1&87.7&68.4&52.1&84.4&91.6&57.4&63.4&77.3&58.1&57.0&53.8&63.8\\
                
                Kosugi \etal\hfilll\cite{Kosugi2019}&85.5&79.6&68.1&55.1&33.6&83.5&83.1&78.5&42.7&79.8&37.8&61.5&74.4&88.6&32.6&55.7&77.9&63.7&78.4&74.1&66.7\\
                
                C-MIL\hfilll\cite{Wan2019}&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&65.0\\
                
                Pred Net\hfilll\cite{Arun2018a}&88.6&86.3&71.8&53.4&51.2&87.6&89.0&65.3&33.2&86.6&58.8&65.9&87.7&93.3&30.9&58.9&83.4&67.8&78.7&80.2&70.9\\
                
                OICR W-RPN\hfilll\cite{Singh}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&66.5\\
                
                SDCN\hfilll\cite{Li2019a}&85.8&83.1&56.2&58.5&44.7&80.2&85.0&77.9&29.6&78.8&53.6&74.2&73.1&88.4&18.2&57.5&74.2&60.8&76.1&79.2&66.8\\
                
                WSOD$^2$\hfilll\cite{Zeng2019}&87.1&80.0&74.8&60.1&36.6&79.2&83.8&70.6&43.5&88.4&46.0&74.7&87.4&90.8&44.2&52.4&81.4&61.8&67.7&79.9&69.5\\
                
                %OICR+GAM+REG \hfilll\cite{Yanga}&81.7&81.2&58.9&54.3&37.8&83.2&86.2&77.0&42.1&83.6&51.3&44.9&78.2&90.8&20.5&56.8&74.2&66.1&81.0&86.0&66.8\\
                PCL+GAM+REG \hfilll\cite{Yanga}&80.0&83.9&74.2&53.2&48.5&82.7&86.2&69.5&39.3&82.9&53.6&61.4&72.4&91.2&22.4&57.5&83.5&64.8&75.7&77.1&68.0\\

                C-MIDN\hfilll\cite{CMIDN}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&68.7\\
                
                OIM+IR\hfilll\cite{Lin2020}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&67.2\\
                
                Ren \etal\hfilll\cite{Ren2020}&87.5&82.4&76.0&58.0&44.7&82.2&87.5&71.2&49.1&81.5&51.7&53.3&71.4&92.8&38.2&52.8&79.4&61.0&78.3&76.0&68.8\\
                
                BOICR\hfilll\cite{Zeni2020}&86.7&73.3&72.4&55.3&46.9&83.2&87.5&64.5&44.6&76.7&46.4&70.9&67.0&88.0&9.6&56.4&69.1&52.4&79.8&82.8&65.7\\
                
                PG-PS\hfilll\cite{Cheng2020}&85.4&80.4&69.1&58.0&35.9&82.7&86.7&82.6&45.5&84.9&44.1&80.2&84.0&89.2&12.3&55.7&79.4&63.4&82.1&82.1&69.2\\

                %==============================================================================================================
                %\hline
                %\multirow{4}{*}{OICR}\hfilll\multirow{4}{*}{\cite{Tang2017}}&81.7&80.4&48.7&49.5&32.8&81.7&85.4&40.1&40.6&79.5&35.7&33.7&60.5&88.8&21.8&57.9&76.3&59.9&75.3&81.4&60.6\\
                %&ResNet18-WS &82.1&60.3&81.1&49.3&67.6&81.4&87.2&84.0&33.4&76.8&21.6&78.8&87.0&87.5&30.8&52.6&81.2&66.6&81.8&82.8&68.7\\
                %&ResNet50-WS &75.9&65.6&70.9&56.9&50.0&81.6&86.8&83.8&33.0&79.5&27.3&79.9&81.7&81.0&30.4&45.0&85.5&72.2&79.1&81.2&67.4\\
                %&ResNet101-WS&83.3&68.6&71.3&53.5&54.7&83.3&88.6&87.3&33.8&80.3&31.6&82.5&85.8&83.8&26.7&42.0&82.5&73.5&80.3&84.7&68.9\\

                %==============================================================================================================
                %\hline
                %\multirow{4}{*}{PCL}\hfilll\multirow{4}{*}{\cite{Tang2018b}}&79.6&85.5&62.2&47.9&37.0&83.8&83.4&43.0&38.3&80.1&50.6&30.9&57.8&90.8&27.0&58.2&75.3&68.5&75.7&78.9&62.7\\
                %&ResNet18-WS   &76.7&81.9&74.4&48.1&53.9&84.5&87.7&86.5&25.4&68.1&36.0&67.4&84.8&86.6&52.5&51.1&81.2&54.9&78.7&62.5&67.1\\
                %&ResNet18-WS F2&79.4&86.2&75.0&54.3&53.2&87.6&88.8&80.9&10.2&81.1&68.0&59.6&89.2&87.5&41.7&59.4&83.3&62.1&80.3&74.2&70.1\\
                %&ResNet50-WS   &75.8&82.7&73.3&48.1&60.4&88.6&88.5&74.2&28.1&71.0&46.3&55.6&88.4&88.3&29.3&56.3&81.2&69.3&79.5&71.8&67.8\\
                %&ResNet101-WS  &84.9&77.2&71.3&60.0&44.8&76.4&86.4&87.9&16.7&86.1&67.0&84.4&86.5&88.8&53.1&50.0&81.3&72.9&85.8&78.9&72.0\\

                %==============================================================================================================
                %\hline
                %\multirow{4}{*}{C-MIL}\hfilll\multirow{4}{*}{\cite{Wan2019}}&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&65.0\\
                %&ResNet18-WS &80.3&64.6&68.3&53.0&56.8&84.5&89.1&86.5&28.1&72.4&28.8&77.3&84.1&79.1&56.8&51.8&85.4&62.1&81.1&80.4&68.5\\
                %&ResNet50-WS &80.8&70.7&74.4&53.4&56.6&85.6&88.0&85.4&35.2&84.2&27.8&78.4&82.4&79.7&31.0&50.0&89.6&73.0&79.1&80.3&69.3\\ %TODO
                %&ResNet101-WS&80.0&77.3&71.6&65.4&54.2&87.3&85.3&83.1&39.8&81.4&46.5&81.9&80.3&87.1&53.8&57.7&87.5&70.9&76.9&81.8&72.4\\ %TODO
                
                %==============================================================================================================
                %\hline
                %\multirow{2}{*}{OICR+GAM+REG}\hfilll\multirow{2}{*}{\cite{Yanga}}&81.7&81.2&58.9&54.3&37.8&83.2&86.2&77.0&42.1&83.6&51.3&44.9&78.2&90.8&20.5&56.8&74.2&66.1&81.0&86.0&66.8\\
                %&ResNet101-WS&92.9&70.7&90.6&69.1&75.5&86.6&90.7&90.8&42.9&88.4&73.2&86.2&97.1&95.0&76.0&60.2&85.4&80.2&89.0&85.2&81.3\\
                
                %==============================================================================================================
                \hline
                \multirow{1}{*}{UWSOD}&98.4&96.8&96.6&98.0&81.9&96.6&96.7&97.1&78.2&98.6&82.5&96.3&97.3&95.2&95.1&80.3&97.9&91.5&98.5&92.1&93.3\\
                %&ResNet18&99.11&94.0&97.2&90.1&86.3&91.8&95.0&96.3&75.5&98.6&89.7&97.0&99.3&95.8&94.0&80.5&100.0&90.1&94.5&87.5&92.6\\
                %&ResNet50&\\ %TODO
                %&ResNet101&\\ %TODO
                
                %====================================================================================================================================================================
                %\hline
                %\multicolumn{22}{c}{Ensemble}\\
                %\hline
                
                %WSDDN Ens.\hfilll\cite{Bilen2016}&&68.9&68.7&65.2&42.5&40.6&72.6&75.2&53.7&29.7&68.1&33.5&45.6&65.9&86.1&27.5&44.9&76.0&62.4&66.3&66.8&58.0\\
                
                %OICR Ens.\hfilll\cite{Tang2017}&&85.4&78.0&61.6&40.4&38.2&82.2&84.2&46.5&15.2&80.1&45.2&41.9&73.8&89.6&18.9&56.0&74.2&62.1&73.0&77.4&61.2\\
                
                %SGWSOD Ens.\hfilll\cite{Lai2017a}&&75.2&78.6&55.8&48.6&45.9&78.5&86.4&65.9&29.4&69.5&34.5&61.1&73.9&85.7&44.2&54.3&77.1&62.5&65.9&78.5&63.6\\
                
                %Ge \etal Ens.\hfilll\cite{Ge}&&75.9&67.6&62.2&37.3&36.6&71.5&80.2&63.8&19.7&70.6&32.4&56.1&67.8&81.7&35.9&50.9&73.4&50.4&66.0&66.8&58.3\\
                
                %CSC Ens.\hfilll\cite{Shen_2019_TIP}&&73.1&76.5&63.9&37.6&52.5&76.9&82.2&71.8&28.5&75.2&40.0&62.2&53.0&80.0&58.8&44.9&77.1&66.8&82.0&71.5&63.7\\
                
                %WSRPN Ens.\hfilll\cite{Tang}&&81.2&81.2&60.7&36.7&52.3&80.7&89.0&65.1&20.5&86.3&61.6&49.5&86.4&92.4&41.4&62.6&79.4&62.4&73.0&75.6&66.9\\
                
                %Pred Net Ens.\hfilll\cite{Arun2018a}&&89.2&86.7&72.2&50.9&51.8&88.3&89.5&65.6&33.6&87.4&59.7&66.4&88.5&94.6&30.4&60.2&83.8&68.9&78.9&81.3&71.4\\
                
                
                %====================================================================================================================================================================
                %\hline
                %\multicolumn{22}{c}{Fast/Faster-RCNN Re-train}\\
                %\hline
                
                %OM+MIL\hfilll\cite{Li2016}&78.2&67.1&61.8&38.1&36.1&61.8&78.8&55.2&28.5&68.8&18.5&49.2&64.1&73.5&21.4&47.4&64.6&22.3&60.9&52.3&52.4\\
                
                %OPG Fast-RCNN\hfilll\cite{Shen_2018_TNNLS}&57.1&44.4&53.9&24.3&11.1&48.9&49.1&70.6&16.0&44.7&38.5&61.5&57.8&65.3&33.3&21.6&50.0&46.3&63.2&32.0&44.5\\
                
                %OICR Ens. Fast-RCNN\hfilll\cite{Tang2017}&85.8&82.7&62.8&45.2&43.5&84.8&87.0&46.8&15.7&82.2&51.0&45.6&83.7&91.2&22.2&59.7&75.3&65.1&76.8&78.1&64.3\\
                
                %W2F \etal \hfilll\cite{Zhang}&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&--&70.3\\
                
                %WSRPN Ens.\hfilll\cite{Tang}&83.8&82.7&60.7&35.1&53.8&82.7&88.6&67.4&22.0&86.3&68.8&50.9&90.8&93.6&44.0&61.2&82.5&65.9&71.1&76.7&68.4\\
                
                %ML-LocNet Ens.\hfilll\cite{Zhang2018g}&81.7&82.9&68.7&44.4&53.9&80.3&88.9&70.5&32.6&74.0&62.7&61.7&81.4&91.6&46.0&60.6&75.2&69.2&78.7&65.8&68.6\\
                
                %CSC Fast-RCNN\hfilll\cite{Shen_2019_TIP}&77.3&81.5&65.8&38.7&59.0&78.0&83.3&73.3&27.2&75.2&47.0&64.9&56.1&86.9&63.7&44.1&76.0&71.2&82.0&70.3&66.1\\
                
                %WS-JDS Fast-RCNN\hfilll\cite{Shen_2019_CVPR}&79.8&84.0&68.3&40.2&61.5&80.5&85.8&75.8&29.7&77.7&49.5&67.4&58.6&87.4&66.2&46.6&78.5&73.7&84.5&72.8&68.6\\
                
                %SD-LocNet\hfilll\cite{Zhang2019b}&76.6&78.0&66.2&47.4&51.8&81.7&86.7&79.6&36.7&72.6&60.0&61.6&80.4&88.8&43.4&54.0&73.9&64.3&78.4&65.1&67.4\\
                %SD-LocNet\hfilll\cite{Zhang2019b}&81.5&83.5&70.0&46.4&52.9&80.1&89.1&73.6&37.3&75.2&73.0&62.5&85.0&91.4&51.3&63.7&79.2&72.9&80.5&68.8&70.9\\
                
                %SDCN Fast-RCNN\hfilll\cite{Li2019a}&88.3&84.3&59.2&58.5&47.7&81.2&86.7&78.8&29.9&81.5&54.0&78.4&75.2&90.8&20.2&55.3&76.3&68.6&79.1&82.8&68.8\\
                
                %C-MIDN FRCNN\hfilll\cite{CMIDN}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&71.9\\
                
                %OIM+IR FRCNN\hfilll\cite{Lin2020}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&68.8\\
                
                %PG-PS FRCNN\hfilll\cite{Cheng2020}&87.1&84.4&70.6&57.7&46.1&85.7&88.1&85.6&46.7&87.2&45.9&83.4&85.6&90.1&18.1&59.7&82.4&68.2&85.3&86.1&72.2\\
                
                %==============================================================================================================
                \hline
            \end{tabular}
        \end{adjustbox}
    \end{center}
    \vspace{-20pt}
    \label{table_voc2007_sota_corloc}
\end{table*}


==> main/table_voc2007_sota_mAP.tex <==
\begin{table*}[t]
    \vspace{-15pt}
    \caption{
        %Comparison with the state-of-the-art methods on PASCAL VOC 2007 in terms of AP (\%) on test set.
        Comparison with the state-of-the-art methods on VOC 2007 in terms of AP on test set.
    }
    \vspace{-10pt}
    \footnotesize
    \begin{center}
        \begin{adjustbox}{max width=1.0\linewidth}
            \begin{tabular}{l|cccccccccccccccccccc|c}
                \hline
                
                Method&aero&bicy&bird&boa&bot&bus&car&cat&cha&cow&dtab&dog&hors&mbik&pers&plnt&she&sofa&trai&tv&Av.\\
                
                \hline
                \multicolumn{22}{c}{Object Mining}\\
                %==============================================================================================================
                \hline
                
                %Song \etal\hfilll\cite{Song2014Weakly}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&24.6\\
                
                %Bilen \etal\hfilll\cite{Bilen2014}&42.2&43.9&23.1&9.2&12.5&44.9&45.1&24.9&8.3&24.0&13.9&18.6&31.6&43.6&7.6&20.9&26.6&20.6&35.9&29.6&26.4\\
                
                %Cover+SLSVM\hfilll\cite{song2014learning}&27.6&41.9&19.7&9.1&10.4&35.8&39.1&33.6&0.6&20.9&10.0&27.7&29.4&39.2&9.1&19.3&20.5&17.1&35.6&7.1&22.7\\
                
                %LCL-pLSA\hfilll\cite{Wang2014}&48.8&41.0&23.6&12.1&11.1&42.7&40.9&35.5&11.1&36.6&18.4&35.3&34.8&51.3&17.2&17.4&26.8&32.8&35.1&45.6&30.9\\
                
                %LCL+Context\hfilll\cite{Wang2014}&48.9&42.3&26.1&11.3&11.9&41.3&40.9&34.7&10.8&34.7&18.8&34.4&35.4&52.7&19.1&17.4&35.9&33.3&34.8&46.5&31.6\\
                
                %Bilen \etal\hfilll\cite{Bilen2015}&46.2&46.9&24.1&16.4&12.2&42.2&47.1&35.2&7.8&28.3&12.7&21.5&30.1&42.4&7.8&20.0&26.8&20.8&35.8&29.6&27.7\\
                
                %Multi-Fold MIL\hfilll\cite{Cinbis2015}&39.3&43.0&28.8&20.4&8.0&45.5&47.9&22.1&8.4&33.5&23.6&29.2&38.5&47.9&20.3&20.0&35.8&30.8&41.0&20.1&30.2\\
                
                %Teh\hfilll\cite{Teh2016}&48.8&45.9&37.4&26.9&9.2&50.7&43.4&43.6&10.6&35.9&27.0&38.6&48.5&43.8&24.7&12.1&29.0&23.2&48.8&41.9&34.5\\
                
                %WSDDN\hfilll\cite{Bilen2016}&42.9&56.0&32.0&17.6&10.2&61.8&50.2&29.0&3.8&36.2&18.5&31.1&45.8&54.5&10.2&15.4&36.3&45.2&50.1&43.8&34.5\\
                %WSDDN\hfilll\cite{Bilen2016}&43.6&50.4&32.2&26.0&9.8&58.5&50.4&30.9&7.9&36.1&18.2&31.7&41.4&52.6&8.8&14.0&37.8&46.9&53.4&47.9&34.9\\
                WSDDN\hfilll\cite{Bilen2016}&39.4&50.1&31.5&16.3&12.6&64.5&42.8&42.6&10.1&35.7&24.9&38.2&34.4&55.6&9.4&14.7&30.2&40.7&54.7&46.9&34.8\\
                
                ContextLocNet\hfilll\cite{Kantorov2016}&57.1&52.0&31.5&7.6&11.5&55.0&53.1&34.1&1.7&33.1&49.2&42.0&47.3&56.6&15.3&12.8&24.8&48.9&44.4&47.8&36.3\\
                
                %Beam Search\hfilll\cite{Bency2016}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&25.7\\
                
                %OM+MIL\hfilll\cite{Li2016}&37.2&35.7&25.8&13.8&12.7&36.2&42.4&22.3&14.3&24.2&9.4&13.1&27.9&38.9&3.7&18.7&20.1&16.3&36.1&18.4&23.4\\
                
                %OPG\hfilll\cite{Shen_2018_TNNLS}&32.5&43.8&20.0&11.6&9.1&42.9&21.0&49.2&4.5&15.2&30.6&29.0&68.9&26.8&9.8&12.4&18.2&28.9&45.7&20.5&27.0\\
                %OPG\hfilll\cite{Shen_2018_TNNLS}&48.9&49.9&25.6&14.0&6.1&47.1&22.5&52.7&3.4&19.6&33.2&33.3&55.3&30.2&9.9&9.1&14.8&25.8&50.8&24.7&28.8\\
                
                WCCN\hfilll\cite{Diba2017}&49.5&60.6&38.6&29.2&16.2&70.8&56.9&42.5&10.9&44.1&29.9&42.2&47.9&64.1&13.8&23.5&45.9&54.1&60.8&54.5&42.8\\
                
                Jie \etal\hfilll\cite{Jie2017}&52.2&47.1&35.0&26.7&15.4&61.3&66.0&54.3&3.0&53.6&24.7&43.6&48.4&65.8&6.6&18.8&51.9&43.6&53.6&62.4&41.7\\
                
                %SPAM-CAM\hfilll\cite{Gudi2017}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&27.5\\
                
                TST\hfilll\cite{Shi2017a}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&33.8\\
                
                %SGWSOD\hfilll\cite{Lai2017a}&45.9&59.6&26.4&24.7&11.4&61.2&56.5&49.3&4.9&35.6&24.1&45.2&56.0&56.5&22.7&19.8&34.7&44.7&50.1&48.3&38.9\\
                %SGWSOD\hfilll\cite{Lai2017a}&VGG-M-1024&45.8&56.1&29.1&26.4&10.5&63.1&59.0&50.3&7.1&34.7&31.4&37.0&49.6&60.1&20.2&17.0&41.3&45.4&51.7&51.7&39.4\\
                SGWSOD\hfilll\cite{Lai2017a}&48.4&61.5&33.3&30.0&15.3&72.4&62.4&59.1&10.9&42.3&34.3&53.1&48.4&65.0&20.5&16.6&40.6&46.5&54.6&55.1&43.5\\
                
                TS$^2$C\hfilll\cite{Wei2018TS2C}&59.3&57.5&43.7&27.3&13.5&63.9&61.7&59.9&24.1&46.9&36.7&45.6&39.9&62.6&10.3&23.6&41.7&52.4&58.7&56.6&44.3\\
                
                %CSC C5\hfilll\cite{Shen_2019_TIP}&46.9&57.5&36.7&14.8&17.5&59.1&51.3&53.0&5.2&39.2&30.1&35.9&50.0&54.2&26.0&19.0&36.6&42.1&62.3&31.0&38.4\\
                %CSC C5\hfilll\cite{Shen_2019_TIP}&45.5&59.4&39.6&15.3&19.9&60.3&53.0&58.1&2.9&38.9&15.5&44.1&45.5&53.6&30.1&19.3&39.3&40.2&60.9&45.5&39.3\\
                %CSC C5\hfilll\cite{Shen_2019_TIP}&51.4&62.0&35.2&18.7&27.9&66.7&53.5&51.4&16.2&43.6&43.0&46.7&20.0&58.4&31.1&23.8&43.6&48.8&65.4&53.5&43.0\\
                
                %WS-JDS\hfilll\cite{Shen_2019_CVPR}&52.0&64.5&45.5&26.7&27.9&60.5&47.8&59.7&13.0&50.4&46.4&56.3&49.6&60.7&25.4&28.2&50.0&51.4&66.5&29.7&45.6\\
                
                %==============================================================================================================
                %\hline
                
                %\multirow{4}{*}{WSDDN}\hfilll\multirow{4}{*}{\cite{Bilen2016}}&39.4&50.1&31.5&16.3&12.6&64.5&42.8&42.6&10.1&35.7&24.9&38.2&34.4&55.6&9.4&14.7&30.2&40.7&54.7&46.9&34.8\\
                %&ResNet18-WS &47.9&56.8&40.2&17.6&29.9&67.2&54.6&49.6&8.7&46.6&47.0&34.8&52.0&61.4&17.0&24.3&42.2&49.3&60.5&59.9&43.4\\
                %&ResNet50-WS &50.4&56.7&41.8&24.9&29.9&64.0&55.8&47.8&21.5&50.3&35.0&49.5&49.5&58.1&13.9&24.5&44.7&40.7&65.3&55.8&44.0\\
                %&ResNet101-WS&47.0&58.6&40.4&21.1&28.4&68.4&57.1&46.5&20.1&49.5&35.5&51.8&48.1&55.8&12.2&19.6&45.4&53.8&63.2&58.1&44.1\\
                
                %\hline
                
                %\multirow{4}{*}{ContextLocNet}\hfilll\multirow{4}{*}{\cite{Kantorov2016}}&57.1&52.0&31.5&7.6&11.5&55.0&53.1&34.1&1.7&33.1&49.2&42.0&47.3&56.6&15.3&12.8&24.8&48.9&44.4&47.8&36.3\\
                %&ResNet18-WS &58.1&56.3&41.6&31.4&22.9&66.1&57.3&64.1&11.0&34.2&45.0&59.7&58.9&60.2&12.9&22.0&30.2&56.6&68.5&50.6&45.4\\
                %&ResNet50-WS &54.9&62.8&41.5&19.1&28.5&67.3&55.1&52.4&17.9&48.3&39.4&45.7&55.3&61.2&31.1&22.2&44.4&46.7&64.6&45.9&45.3\\ %TODO
                %&ResNet101-WS&60.6&53.5&50.3&26.1&26.4&66.9&55.8&73.1&18.0&35.7&19.2&54.7&56.0&65.6&25.5&24.3&30.3&51.9&69.4&54.4&45.9\\ %TODO
                
                %==============================================================================================================
                \hline
                \multicolumn{22}{c}{Object Mining + Instance Refinement}\\
                \hline
                
                %OICR\hfilll\cite{Tang2017}&53.1&57.1&32.4&12.3&15.8&58.2&56.7&39.6&0.9&44.8&39.9&31.0&54.0&62.4&4.5&20.6&39.2&38.1&48.9&48.6&37.9\\
                OICR\hfilll\cite{Tang2017}&58.0&62.4&31.1&19.4&13.0&65.1&62.2&28.4&24.8&44.7&30.6&25.3&37.8&65.5&15.7&24.1&41.7&46.9&64.3&62.6&41.2\\
                
                %K-EM\hfilll\cite{Yan2017}&59.8&64.6&47.8&28.8&21.4&67.7&70.3&61.2&17.2&51.5&34.0&42.3&48.8&65.9&9.3&21.1&53.6&51.4&54.7&50.7&46.1\\
                
                MELM\hfilll\cite{Wan}&55.6&66.9&34.2&29.1&16.4&68.8&68.1&43.0&25.0&65.6&45.3&53.2&49.6&68.6&2.0&25.4&52.5&56.8&62.1&57.1&47.3\\
                
                ZLDN\hfilll\cite{Zhang2018b}&55.4&68.5&50.1&16.8&20.8&62.7&66.8&56.5&2.1&57.8&47.5&40.1&69.7&68.2&21.6&27.2&53.4&56.1&52.5&58.2&47.6\\
                
                %GAL-fWSD300\hfilll\cite{Shen_2018_CVPR}&52.0&60.5&44.6&26.1&20.6&63.1&66.2&65.3&15.0&50.1&52.8&56.7&21.3&63.4&36.8&22.7&47.9&51.7&68.9&54.1&47.0\\
                %GAL-fWSD512\hfilll\cite{Shen_2018_CVPR}&58.4&63.8&45.8&24.0&22.7&67.7&65.7&58.9&15.0&58.1&47.0&53.7&23.8&64.3&36.2&22.3&46.7&50.3&70.8&55.1&47.5\\
                
                %ML-LocNet\hfilll\cite{Zhang2018g}&VGG-S&57.0&64.0&42.6&22.1&17.9&59.3&64.0&39.5&2.2&47.6&55.0&38.9&66.4&68.1&30.6&23.5&43.2&44.1&55.4&46.3&44.4\\
                %ML-LocNet\hfilll\cite{Zhang2018g}&57.2&64.6&44.5&26.3&21.1&65.7&67.1&56.4&16.1&51.7&50.5&37.2&64.2&69.4&24.5&25.4&51.9&51.3&56.9&42.2&47.2\\
                ML-LocNet\hfilll\cite{Zhang2018g}&59.3&68.9&45.7&29.0&24.5&64.8&68.4&59.3&18.6&49.1&50.2&43.1&65.8&70.2&19.9&24.3&48.1&54.2&62.8&41.8&48.4\\
                
                WSRPN\hfilll\cite{Tang}&57.9&70.5&37.8&5.7&21.0&66.1&69.2&59.4&3.4&57.1&57.3&35.2&64.2&68.6&32.8&28.6&50.8&49.5&41.1&30.0&45.3\\
                
                PCL\hfilll \cite{Tang2018b}&54.4&69.0&39.3&19.2&15.7&62.9&64.4&30.0&25.1&52.5&44.4&19.6&39.3&67.7&17.8&22.9&46.6&57.5&58.6&63.0&43.5\\
                
                Kosugi \etal\hfilll\cite{Kosugi2019}&61.5&64.8&43.7&26.4&17.1&67.4&62.4&67.8&25.4&51.0&33.7&47.6&51.2&65.2&19.3&24.4&44.6&54.1&65.6&59.5&47.6\\
                
                %C-MIL\hfilll\cite{Wan2019}&54.5&55.5&34.4&20.3&16.7&53.4&59.2&44.6&8.4&46.0&40.2&40.8&47.7&63.2&22.8&23.2&39.4&44.3&53.8&52.3&40.7\\
                C-MIL\hfilll\cite{Wan2019}&62.5&58.4&49.5&32.1&19.8&70.5&66.1&63.4&20.0&60.5&52.9&53.5&57.4&68.9&8.4&24.6&51.8&58.7&66.7&63.5&50.5\\
                
                Pred Net\hfilll\cite{Arun2018a}&66.7&69.5&52.8&31.4&24.7&74.5&74.1&67.3&14.6&53.0&46.1&52.9&69.9&70.8&18.5&28.4&54.6&60.7&67.1&60.4&52.9\\
                
                WSDDN + W-RPN\hfilll\cite{Singh}&55.9&52.6&27.4&20.7&7.8&63.6&54.8&55.7&4.9&37.6&35.6&59.4&52.0&54.8&19.6&12.9&31.9&44.2&57.4&39.2&39.4\\
                OICR W-RPN\hfilll\cite{Singh}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&46.9\\
                
                SDCN\hfilll\cite{Li2019a}&59.8&67.1&32.0&34.7&22.8&67.1&63.8&67.9&22.5&48.9&47.8&60.5&51.7&65.2&11.8&20.6&42.1&54.7&60.8&64.3&48.3\\
                
                WSOD$^2$\hfilll\cite{Zeng2019}&65.1&64.8&57.2&39.2&24.3&69.8&66.2&61.0&29.8&64.6&42.5&60.1&71.2&70.7&21.9&28.1&58.6&59.7&52.2&64.8&53.6\\
                
                %OICR+GAM+REG \hfilll\cite{Yanga}&55.2&66.5&40.1&31.1&16.9&69.8&64.3&67.8&27.8&52.9&47.0&33.0&60.8&64.4&13.8&26.0&44.0&55.7&68.9&65.5&48.6\\
                PCL+GAM+REG \hfilll\cite{Yanga}&57.6&70.8&50.7&28.3&27.2&72.5&69.1&65.0&26.9&64.5&47.4&47.7&53.5&66.9&13.7&29.3&56.0&54.9&63.4&65.2&51.5\\
                
                C-MIDN\hfilll\cite{CMIDN}&53.3&71.5&49.8&26.1&20.3&70.3&69.9&68.3&28.7&65.3&45.1&64.6&58.0&71.2&20.0&27.5&54.9&54.9&69.4&63.5&52.6\\
                
                %OIM\hfilll\cite{Lin2020}&62.2&67.2&48.0&29.6&23.5&68.7&69.3&64.3&22.8&59.6&39.6&30.7&42.7&69.8&3.1&23.3&57.9&55.4&63.4&63.5&48.2\\
                OIM+IR\hfilll\cite{Lin2020}&55.6&67.0&45.8&27.9&21.1&69.0&68.3&70.5&21.3&60.2&40.3&54.5&56.5&70.1&12.5&25.0&52.9&55.2&65.0&63.7&50.1\\
                
                Ren \etal\hfilll\cite{Ren2020}&68.8&77.7&57.0&27.7&28.9&69.1&74.5&67.0&32.1&73.2&48.1&45.2&54.4&73.7&35.0&29.3&64.1&53.8&65.3&65.2&54.9\\
                
                BOICR\hfilll\cite{Zeni2020}&68.6&62.4&55.5&27.2&21.4&71.1&71.6&56.7&24.7&60.3&47.4&56.1&46.4&69.2&2.7&22.9&41.5&47.7&71.1&69.8&49.7\\
                
                PG-PS\hfilll\cite{Cheng2020}&63.0&64.4&50.1&27.5&17.1&70.6&66.0&71.1&25.8&55.9&43.2&62.7&65.9&64.1&10.2&22.5&48.1&53.8&72.2&67.4&51.1\\
                
                %==============================================================================================================
                %\hline
                %\multirow{4}{*}{OICR}\hfilll\multirow{4}{*}{\cite{Tang2017}}&58.0&62.4&31.1&19.4&13.0&65.1&62.2&28.4&24.8&44.7&30.6&25.3&37.8&65.5&15.7&24.1&41.7&46.9&64.3&62.6&41.2\\
                %&ResNet18-WS &61.3&54.5&52.4&30.1&34.9&68.9&65.0&75.0&22.5&57.4&19.7&66.6&64.8&64.9&16.8&22.3&53.2&54.9&69.9&64.8&51.0\\
                %&ResNet50-WS &61.2&50.9&55.0&33.2&36.2&68.6&65.7&79.2&17.3&58.1&19.3&69.1&65.7&64.8&15.1&18.9&50.1&55.1&69.8&64.4&50.9\\
                %&ResNet101-WS&63.2&51.1&51.9&33.7&32.4&67.9&65.0&78.9&19.0&59.4&21.9&70.6&68.3&64.4&15.2&20.8&49.3&55.3&72.5&66.6&51.4\\
                
                %==============================================================================================================
                %\hline
                %\multirow{4}{*}{PCL}\hfilll\multirow{4}{*}{\cite{Tang2018b}}&54.4&69.0&39.3&19.2&15.7&62.9&64.4&30.0&25.1&52.5&44.4&19.6&39.3&67.7&17.8&22.9&46.6&57.5&58.6&63.0&43.5\\
                %&ResNet18-WS   &54.4&69.5&48.7&29.7&33.2&70.7&69.7&57.2&11.5&62.4&37.2&39.3&66.3&67.5&23.7&30.9&60.1&52.0&65.3&55.3&50.2\\
                %&ResNet18-WS F2&54.5&67.6&48.1&31.6&32.6&71.5&72.3&67.7&3.3&64.2&58.7&45.4&67.3&68.4&27.7&30.8&56.7&50.6&67.4&51.1&51.9\\
                %&ResNet50-WS   &55.4&60.7&50.8&30.1&31.0&69.8&69.0&66.6&9.6&62.0&25.0&56.4&68.2&65.5&35.7&28.1&57.2&52.9&67.0&54.2&50.8\\
                %&ResNet101-WS  &57.5&66.4&55.2&28.8&31.2&71.8&68.5&76.8&3.2&61.4&57.0&69.0&71.6&66.4&36.8&24.1&54.1&54.0&71.7&61.4&54.3\\
                
                %==============================================================================================================
                %\hline
                %\multirow{4}{*}{C-MIL}\hfilll\multirow{4}{*}{\cite{Wan2019}}&62.5&58.4&49.5&32.1&19.8&70.5&66.1&63.4&20.0&60.5&52.9&53.5&57.4&68.9&8.4&24.6&51.8&58.7&66.7&63.5&50.5\\
                %&ResNet18-WS &57.0&54.9&43.6&39.9&32.2&70.9&69.8&75.2&14.2&59.9&28.5&66.3&67.5&65.3&37.6&21.8&56.7&49.8&71.1&68.9&52.6\\
                %&ResNet50-WS &67.5&45.2&62.9&33.4&41.6&73.9&66.7&76.2&26.4&54.8&11.6&71.4&71.9&72.9&20.6&31.9&42.5&58.8&77.1&61.3&53.4\\ %TODO
                %&ResNet101-WS&68.7&43.4&66.7&37.5&44.2&75.7&69.3&78.3&25.4&58.0&14.1&70.7&76.5&77.1&24.6&36.1&45.6&62.5&78.2&66.2&55.9\\ %TODO
                
                %==============================================================================================================
                %\hline
                %\multirow{2}{*}{OICR+GAM+REG}\hfilll\multirow{2}{*}{\cite{Yanga}}&55.2&66.5&40.1&31.1&16.9&69.8&64.3&67.8&27.8&52.9&47.0&33.0&60.8&64.4&13.8&26.0&44.0&55.7&68.9&65.5&48.6\\
                %&ResNet101-WS&68.8&54.6&66.6&44.7&34.4&72.1&70.8&80.0&21.7&63.2&57.7&72.8&79.9&73.2&51.9&23.5&55.7&60.4&75.3&62.0&59.5\\
                
                %==============================================================================================================
                \hline
                \multirow{1}{*}{UWSOD}&74.0&77.6&66.2&57.8&51.0&78.0&74.7&81.5&43.2&70.5&67.6&77.8&81.2&71.1&67.7&36.7&59.0&66.1&78.6&72.0&67.7\\
                %&ResNet18&74.4&79.4&69.7&59.9&52.7&77.8&75.7&83.8&45.1&74.6&68.6&81.8&82.5&73.1&66.2&33.9&64.3&62.1&75.5&73.4&68.7\\
                %&ResNet50&\\ %TODO
                %&ResNet101&\\ %TODO
                
                \hline
                \multicolumn{22}{c}{FSOD}\\
                \hline
                
                Fast RCNN\hfilll\cite{FASTRCNN}&74.5&78.3&69.2&53.2&36.6&77.3&78.2&82.0&40.7&72.7&67.9&79.6&79.2&73.0&69.0&30.1&65.4&70.2&75.8&65.8&66.9\\
                Faster RCNN\hfilll\cite{FASTERRCNN}&70.0&80.6&70.1&57.3&49.9&78.2&80.4&82.0&52.2&75.3&67.2&80.3&79.8&75.0&76.3&39.1&68.3&67.3&81.1&67.6&69.9\\
                
                %====================================================================================================================================================================
                %\hline
                %\multicolumn{22}{c}{Ensemble}\\
                %\hline

                %WSDDN Ens.\hfilll\cite{Bilen2016}&&46.4&58.3&35.5&25.9&14.0&66.7&53.0&39.2&8.9&41.8&26.6&38.6&44.7&59.0&10.8&17.3&40.7&49.6&56.9&50.8&39.3\\
                
                %OICR Ens.\hfilll\cite{Tang2017}&&58.5&63.0&35.1&16.9&17.4&63.2&60.8&34.4&8.2&49.7&41.0&31.3&51.9&64.8&13.6&23.1&41.6&48.4&58.9&58.7&42.0\\
                
                %SGWSOD Ens.\hfilll\cite{Lai2017a}&&48.5&63.2&33.2&31.0&14.5&69.4&61.7&56.6&8.5&41.3&37.6&50.0&54.1&62.7&22.9&20.6&42.1&50.7&54.3&55.2&43.9\\
                
                %Ge \etal Ens.\hfilll\cite{Ge}&&49.1&53.6&43.5&21.3&18.5&66.9&64.0&55.6&11.9&53.7&26.6&45.6&48.7&64.6&20.4&23.3&50.0&44.7&55.9&60.6&43.9\\
                
                %CSC Ens.\hfilll\cite{Shen_2019_TIP}&&49.4&63.6&40.6&16.7&26.3&65.1&55.7&57.8&9.3&45.1&37.1&47.5&32.6&57.2&33.6&24.0&43.2&47.9&64.1&53.1&43.5\\
                
                %WSRPN Ens.\hfilll\cite{Tang}&&60.3&66.2&45.0&19.6&26.6&68.1&68.4&49.4&8.0&56.9&55.0&33.6&62.5&68.2&20.6&29.0&49.0&54.1&58.8&58.4&47.9\\
                
                %Pred Net Ens.\hfilll\cite{Arun2018a}&&67.7&70.4&52.9&31.3&26.1&75.5&73.7&68.6&14.9&54.0&47.3&53.7&70.8&70.2&19.7&29.2&54.9&61.3&67.6&61.2&53.6\\
                
                %MIL+GAM+REG-Ens. \hfilll\cite{Yanga}&&59.8&72.8&54.4&35.6&30.2&74.4&70.6&74.5&27.7&68.0&51.7&46.3&63.7&68.6&14.8&27.8&54.9&60.9&65.1&67.4&54.5\\

                %====================================================================================================================================================================
                %\hline
                %\multicolumn{22}{c}{Fast/Faster-RCNN Re-train}\\
                %\hline
                
                %OM+MIL\hfilll\cite{Li2016}&54.5&47.4&41.3&20.8&17.7&51.9&63.5&46.1&21.8&57.1&22.1&34.4&50.5&61.8&16.2&29.9&40.7&15.9&55.3&40.2&39.5\\
                
                %OPG Fast-RCNN\hfilll\cite{Shen_2018_TNNLS}&40.3&38.6&34.0&17.6&1.7&43.2&34.6&57.5&10.5&19.6&32.9&50.3&43.1&44.3&11.2&5.8&28.0&35.2&56.4&23.8&31.4\\
                
                %OICR Ens. Fast-RCNN\hfilll\cite{Tang2017}&65.5&67.2&47.2&21.6&22.1&68.0&68.5&35.9&5.7&63.1&49.5&30.3&64.7&66.1&13.0&25.6&50.0&57.1&60.2&59.0&47.0\\
                
                %Ge \etal\hfilll\cite{Ge2018}&64.3&68.0&56.2&36.4&23.1&68.5&67.2&64.9&7.1&54.1&47.0&57.0&69.3&65.4&20.8&23.2&50.7&59.6&65.2&57.0&51.2\\
                
                %W2F \etal\hfilll\cite{Zhang}&63.5&70.1&50.5&31.9&14.4&72.0&67.8&73.7&23.3&53.4&49.4&65.9&57.2&67.2&27.6&23.8&51.8&58.7&64.0&62.3&52.4\\
                
                %TS$^2$C\hfilll\cite{Wei2018TS2C}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&48.0\\
                
                %WSRPN Ens.\hfilll\cite{Tang}&63.0&69.7&40.8&11.6&27.7&70.5&74.1&58.5&10.0&66.7&60.6&34.7&75.7&70.3&25.7&26.5&55.4&56.4&55.5&54.9&50.4\\
                
                %ML-LocNet\hfilll\cite{Zhang2018g}&60.8&70.6&47.8&30.2&24.8&64.9&68.4&57.9&11.0&51.3&55.5&48.1&68.7&69.5&28.3&25.2&51.3&56.5&60.0&43.1&49.7\\
                
                %CSC Fast-RCNN\hfilll\cite{Shen_2019_TIP}&58.4&63.3&48.1&21.7&29.6&66.7&66.3&66.1&9.3&61.1&40.5&49.5&35.9&64.9&39.2&26.4&53.2&55.6&70.2&54.0&49.0\\
                
                %WS-JDS Fast-RCNN\hfilll\cite{Shen_2019_CVPR}&64.8&70.7&51.5&25.1&29.0&74.1&69.7&69.6&12.7&69.5&43.9&54.9&39.3&71.3&32.6&29.8&57.0&61.0&66.6&57.4&52.5\\
                
                %SD-LocNet\hfilll\cite{Zhang2019b}&59.2&67.2&46.1&29.6&21.6&65.7&68.0&61.4&17.3&53.1&50.6&38.3&67.7&69.1&26.8&25.1&49.2&52.2&60.9&39.6&48.4\\
                %SD-LocNet\hfilll\cite{Zhang2019b}&65.1&72.5&50.3&31.3&24.2&68.3&70.9&65.1&19.0&51.0&53.4&47.5&70.2&69.9&25.9&25.6&45.8&57.9&71.2&40.9&51.3\\
                
                %Kosugi \etal Fast-RCNN\hfilll\cite{Kosugi2019}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&51.4\\
                %Kosugi \etal PGE Fast-RCNN\hfilll\cite{Kosugi2019}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&52.1\\
                
                %C-MIL Fast-RCNN\hfilll\cite{Wan2019}&61.8&60.9&56.2&28.9&18.9&68.2&69.6&71.4&18.5&64.3&57.2&66.9&65.9&65.7&13.8&22.9&54.1&61.9&68.2&66.1&53.1\\
                
                %SDCN Fast-RCNN\hfill \cite{Li2019a}&61.1&70.6&40.2&32.8&23.9&63.4&68.9&68.2&18.3&60.2&53.5&63.6&53.6&66.1&14.6&21.8&50.5&56.9&62.4&67.9&51.0\\
                
                %C-MIDN FRCNN\hfilll\cite{CMIDN}&54.1&74.5&56.9&26.4&22.2&68.7&68.9&74.8&25.2&64.8&46.4&70.3&66.3&67.5&21.6&24.4&53.0&59.7&68.7&58.9&53.6\\
                
                %OIM+IR FRCNN \hfilll\cite{Lin2020}&53.4&72.0&51.4&26.0&27.7&69.8&69.7&74.8&21.4&67.1&45.7&63.7&63.7&67.4&10.9&25.3&53.5&60.4&70.8&58.1&52.6\\
                
                %BOICR FRCNN\hfilll\cite{Zeni2020}&65.8&58.6&55.0&32.4&19.5&74.2&71.4&70.9&19.2&54.8&46.2&67.5&57.0&65.6&1.4&16.7&40.4&53.0&69.5&61.1&50.0\\
                
                %PG-PS FRCNN\hfilll\cite{Cheng2020}&59.3&66.2&55.4&35.2&22.3&69.7&70.2&73.8&29.4&63.6&47.9&78.1&67.9&68.2&12.2&24.9&43.2&63.7&73.2&66.8&54.6\\
                
                %==============================================================================================================
                \hline
            \end{tabular}
        \end{adjustbox}
    \end{center}
    \vspace{-15pt}
    \label{table_voc2007_sota_map}
\end{table*}


==> main/table_voc2007voc2012mscoco_sota_net.tex <==
\begin{table*}[t]
%    \vspace{-20pt}
    \caption{
        Comparison with the state-of-the-art methods on PASCAL VOC 2007, 2012 and MS COCO.
%        \scriptsize{
        %    $^{\ddag}$\url{http://host.robots.ox.ac.uk:8080/anonymous/3ESVLJ.html}
        %    $^{\P}$\url{http://host.robots.ox.ac.uk:8080/anonymous/FUTRJO.html}
        %    $^{\$}$\url{http://host.robots.ox.ac.uk:8080/anonymous/ICYSCH.html}
        %    $^{\dag}$\url{http://host.robots.ox.ac.uk:8080/anonymous/WOPMN0.html}
        %    $^{\S}$\url{http://host.robots.ox.ac.uk:8080/anonymous/LX5460.html}
        %    $^{\pounds}$\url{http://host.robots.ox.ac.uk:8080/anonymous/NNFS4F.html}
%        }
    }
    %\vspace{-10pt}
    %\footnotesize
    \begin{center}
        \begin{adjustbox}{max width=1.0\textwidth}
            \begin{tabular}{l|c|cc|cc|ccc}
                \toprule

                \multirow{3}{*}{Method}&\multirow{3}{*}{Bakcbone}&\multicolumn{2}{c|}{PASCAL VOC 2007}&\multicolumn{2}{c|}{PASCAL VOC 2012}&\multicolumn{3}{c}{MS COCO}\\

                &&\multirow{2}{*}{$m$AP (\%)}&\multirow{2}{*}{CorLoc (\%)}&\multirow{2}{*}{$m$AP (\%)}&\multirow{2}{*}{CorLoc (\%)}&\multicolumn{3}{c}{Avg. Precision, IoU:}\\

                &&&&&&0.5:0.95&0.5&0.75\\

                \midrule
                \multicolumn{9}{c}{WSOD {with} external object proposal modules or additional data}\\
                \midrule%==============================================================================================================

%                \multicolumn{9}{c}{Object Discovery}\\
%                \hline

%                Siva \etal\hfilll\cite{siva2012defence}&&--&30.2&--&--&--&--&--\\

%                Shi \etal\hfilll\cite{Shi2017}&&--&36.2&--&--&--&--&--\\

%                Rochan \etal\hfilll\cite{Rochan2015}&AlexNet&--&58.8&--&--&--&--&--\\

%                RMI-SVM\hfilll\cite{Wang2015}&AlexNet&--&40.2&--&--&--&--&--\\

%                STL\hfilll\cite{Bazzani2016}&AlexNet&--&54.4&--&--&--&--&--\\

%                Song \etal\hfilll\cite{Song2014Weakly}&AlexNet&24.6&--&--&--&--&--&--\\

%                Bilen \etal\hfilll\cite{Bilen2014}&AlexNet&26.4&--&--&--&--&--&--\\

%                Cover+SLSVM\hfilll\cite{song2014learning}&AlexNet&22.7&--&--&--&--&--&--\\

%                LCL-pLSA\hfilll\cite{Wang2014}&AlexNet&30.9&48.5&--&--&--&--&--\\
%                LCL+Context\hfilll\cite{Wang2014}&AlexNet&31.6&--&--&--&--&--&--\\

%                Bilen \etal\hfilll\cite{Bilen2015}&AlexNet&27.7&43.7&--&--&--&--&--\\

                Multi-Fold MIL\hfilll\cite{Cinbis2015}&AlexNet&30.2&52.0&--&--&--&--&--\\

%                Teh\hfilll\cite{Teh2016}&AlexNet&34.5&64.6&--&--&--&--&--\\

%                WSDDN\hfilll\cite{Bilen2016}&VGG-F&34.5&54.2&--&--&--&--&--\\
%                WSDDN\hfilll\cite{Bilen2016}&VGG-M&34.9&56.1&--&--&--&--&--\\
                WSDDN\hfilll\cite{Bilen2016}&VGG16&34.8&53.5&--&--&9.5&19.2&8.2\\

                ContextLocNet\hfilll\cite{Kantorov2016}&VGG-F&36.3&55.1&35.3&54.8&11.1&22.1&10.7\\

%                Beam Search\hfilll\cite{Bency2016}&VGG16&25.7&--&26.5&--&--&--&--\\

%                OM+MIL\hfilll\cite{Li2016}&AlexNet&23.4&41.2&29.1&--&--&--&--\\

%                OPG\hfilll\cite{Shen2018OPG}&AlexNet&27.0&34.2&--&--&--&--&--\\
%                OPG\hfilll\cite{Shen2018OPG}&VGG16&28.8&43.5&--&--&--&--&--\\

                WCCN\hfilll\cite{Diba2017}&VGG16&42.8&56.7&37.9&--&--&--&--\\

%                Jiang \etal\hfilll\cite{Jiang2017}&AlexNet&37.4&57.3&33.6&--&--&--&--\\

                Jie \etal\hfilll\cite{Jie2017}&VGG16&41.7&56.1&38.3&58.8&--&--&--\\

%                SPAM-CAM\hfilll\cite{Gudi2017}&VGG16&27.5&--&--&--&--&--&--\\

                TST\hfilll\cite{Shi2017a}&AlexNet&33.8&59.5&--&--&--&--&--\\

%                SGWSOD\hfilll\cite{Lai2017a}&VGG-F&38.9&60.8&--&--&--&--&--\\
%                SGWSOD\hfilll\cite{Lai2017a}&VGG-M-1024&39.4&59.6&--&--&--&--&--\\
                SGWSOD\hfilll\cite{Lai2017a}&VGG16&43.5&62.9&39.6&62.9&--&--&--\\

                TS$^2$C\hfilll\cite{Wei2018TS2C}&VGG16&44.3&61.0&40.0&64.4&--&--&--\\

%                CSC C5\hfilll\cite{Shen2019CSC}&VGG-F&38.4&60.4&--&--&--&--&--\\
%                CSC C5\hfilll\cite{Shen2019CSC}&VGG-M&39.3&60.6&--&--&--&--&--\\
                CSC C5\hfilll\cite{Shen2019CSC}&VGG16&43.0&62.2&37.1&61.4&12.9&23.8&13.2\\

                WS-JDS\hfilll\cite{Shen2019WSJDS}&VGG16&45.6&64.5&39.1&63.5&--&--&--\\

                Oquab \etal\hfilll\cite{Oquab2015}&AlexNet&--&--&11.7&--&--&--&--\\

%                \hline%==============================================================================================================

%                \multirow{4}{*}{WSDDN}\hfilll\multirow{4}{*}{\cite{Bilen2016}}&VGG16&34.8&53.5&--&--\\
%                &ResNet18-WS&43.4&63.1&--&--\\
%                &ResNet50-WS&44.0&63.6&--&--\\
%                &ResNet101-WS&44.1&64.0&--&--\\
%
%                \hline%==============================================================================================================
%
%                \multirow{4}{*}{ContextLocNet}\hfilll\multirow{4}{*}{\cite{Kantorov2016}}&VGG-F&36.3&55.1&35.3&54.8\\
%                &ResNet18-WS&45.4&64.7&42.0$^{\ddag}$&66.7\\
%                &ResNet50-WS&45.3&65.1&--&--\\ %TODO
%                &ResNet101-WS&45.9&65.7&--&--\\ %TODO
%
%                \hline%==============================================================================================================

%                \multicolumn{9}{c}{Object Discovery + Instance Refinement}\\
%                \hline

%                OICR\hfilll\cite{Tang2017}&VGG-M&37.9&57.3&34.6&60.7&--&--&--\\
                OICR\hfilll\cite{Tang2017}&VGG16&41.2&60.6&37.9&62.1&--&--&--\\

                K-EM\hfilll\cite{Yan2017}&VGG16&46.1&65.0&--&--&--&--&--\\

                MELM\hfilll\cite{Wan}&VGG16&47.3&61.4&42.4&--&--&--&--\\

                ZLDN\hfilll\cite{Zhang2018b}&VGG16&47.6&61.2&42.9&61.5&--&--&--\\

%                GAL-fWSD300\hfilll\cite{Shen2018GAL}&VGG16&47.0&68.1&43.1&67.2&--&--&--\\
                GAL-fWSD512\hfilll\cite{Shen2018GAL}&VGG16&47.5&66.1&--&--&--&--&--\\

%                ML-LocNet\hfilll\cite{Zhang2018g}&VGG-S&44.4&63.7&--&--&--&--&--\\
%                ML-LocNet\hfilll\cite{Zhang2018g}&VGG-M&47.2&65.3&--&--&--&--&--\\
                ML-LocNet\hfilll\cite{Zhang2018g}&VGG16&48.4&67.0&42.2&66.3&--&16.2&--\\

                WSRPN\hfilll\cite{Tang}&VGG16&45.3&63.8&40.8&64.9&--&--&--\\

                PCL\hfilll \cite{Tang2018b}&VGG16&43.5&--&--&--&8.5&19.4&--\\

                Kosugi \etal\hfilll\cite{Kosugi2019}&VGG16&47.6&66.7&43.4&66.7&--&--&--\\

%                C-MIL\hfilll\cite{Wan2019}&VGG-F&40.7&--&--&--&--&--&--\\
                C-MIL\hfilll\cite{Wan2019}&VGG16&50.5&65.0&46.7&67.4&--&--&--\\

                Pred Net\hfilll\cite{Arun2018a}&VGG16&52.9&70.9&48.4&69.5&--&--&--\\

%                WSDDN + W-RPN\hfilll\cite{Singh}&VGG16&39.4&--&--&--&--&--&--\\
                OICR W-RPN\hfilll\cite{Singh}&VGG16&46.9&--&43.2&67.5&--&--&--\\

                SDCN\hfilll\cite{Li2019a}&VGG16&48.3&66.8&43.5&67.9&--&--&--\\

                Sona \etal\hfilll\cite{Sona}&VGG16&45.4&--&--&--&--&--&--\\

                WSOD$^2$\hfilll\cite{Zeng2019}&VGG16&53.6&69.5&47.2&\textbf{71.9}&10.8&22.7&--\\

                OICR+GAM+REG \hfilll\cite{Yanga}&VGG16&48.6&66.8&--&--&--&--&--\\
%                PCL+GAM+REG \hfilll\cite{Yanga}&VGG16&51.5&68.0&--&--&--&--&--\\

                C-MIDN\hfilll\cite{CMIDN}&VGG16&52.6&68.7&50.2&71.2&9.6&21.4&--\\

%                OIM\hfilll\cite{Lin2020}&VGG16&48.2&--&--&--&--&--&--\\
                OIM+IR\hfilll\cite{Lin2020}&VGG16&50.1&67.2&45.3&67.1&--&--&--\\

                Ren \etal\hfilll\cite{Ren2020}&VGG16&\textbf{54.9}&68.8&\textbf{52.1}&70.9&12.4&25.8&10.5\\

                Zeni \etal\hfilll\cite{Zeni2020}&VGG16&49.7&65.7&--&66.3&--&--&--\\

                PG-PS\hfilll\cite{Cheng2020}&VGG16&51.1&\textbf{69.2}&48.3&68.7&--&20.7&--\\

                \midrule
                \multicolumn{9}{c}{WSOD {without} external object proposal modules or additional data}\\
                \midrule%==============================================================================================================

                Shi \etal\hfilll\cite{Shi2017}&--&--&36.2&--&--&--&--&--\\

                Beam Search\hfilll\cite{Bency2016}&VGG16&25.7&--&26.5&--&--&--&--\\

                OM+MIL\hfilll\cite{Li2016}&AlexNet&23.4&41.2&29.1&--&--&--&--\\

                %OPG\hfilll\cite{Shen2018OPG}&AlexNet&27.0&34.2&--&--&--&--&--\\
                OPG\hfilll\cite{Shen2018OPG}&VGG16&28.8&43.5&--&--&--&--&--\\

                SPAM-CAM\hfilll\cite{Gudi2017}&VGG16&27.5&--&--&--&--&--&--\\

                \midrule
                \multirow{2}{*}{UWSOD}&VGG16&44.0&63.0&45.1&65.2&2.5&9.3&1.1\\
                &WSR18&\textbf{45.0}&\textbf{63.8}&\textbf{46.2}&\textbf{65.7}&3.1&10.1&1.4\\

%                \midrule%==============================================================================================================
%
%                \multirow{4}{*}{OICR}\hfilll\multirow{4}{*}{\cite{Tang2017}}&VGG16&41.2&60.6&37.9&62.1\\
%                &ResNet18-WS&51.0&68.7&&\\
%                &ResNet50-WS&50.9&67.4&50.4$^{\P}$&72.5\\
%                &ResNet101-WS&51.4&68.9&48.6$^{\$}$&70.3\\
%
%                \hline%==============================================================================================================
%
%                \multirow{4}{*}{PCL}\hfilll\multirow{4}{*}{\cite{Tang2018b}}&VGG16&43.5&62.7&40.6&63.2\\
%                &ResNet18-WS&50.2&67.1&--&--\\
%                &ResNet18-WS F2&51.9&70.1&--&--\\
%                &ResNet50-WS&50.8&67.8&--&--\\
%                &ResNet101-WS&54.3&72.0&51.2$^{\dag}$&73.5\\
%
%                \hline%==============================================================================================================
%
%                \multirow{4}{*}{C-MIL}\hfilll\multirow{4}{*}{\cite{Wan2019}}&VGG16&50.5&65.0&46.7&67.4\\
%                &ResNet18-WS&52.6&68.5&50.6$^{\S}$&73.0\\
%                &ResNet50-WS&53.4&69.3&--&--\\ %TODO
%                &ResNet101-WS&55.9&72.4&--&--\\ %TODO
%
%                \hline%==============================================================================================================
%
%                \multirow{2}{*}{OICR+GAM+REG}\hfilll\multirow{2}{*}{\cite{Yanga}}&VGG16&48.6&66.8&46.8&69.5\\
%                &ResNet101-WS&59.5&81.3&59.1$^{\pounds}$&81.0\\
%
%                \hline%==============================================================================================================
%
%                \multicolumn{9}{c}{Ensemble}\\
%                \hline
%                WSDDN Ens.\hfilll\cite{Bilen2016}&&39.3&58.0&--&--\\
%
%                OICR Ens.\hfilll\cite{Tang2017}&&42.0&61.2&38.2&63.5\\
%
%                SGWSOD Ens.\hfilll\cite{Lai2017a}&&43.9&63.6&40.6&64.2\\
%
%                Ge \etal Ens.\hfilll\cite{Ge}&&43.9&58.3&--&--\\
%
%                CSC Ens.\hfilll\cite{Shen2019CSC}&&43.5&63.7&--&--\\
%
%                WSRPN Ens.\hfilll\cite{Tang}&&47.9&66.9&43.4&67.2\\
%
%                Pred Net Ens.\hfilll\cite{Arun2018a}&&53.6&71.4&49.5&70.2\\
%
%                MIL+GAM+REG-Ens. \hfilll\cite{Yanga}&&54.5&--&--&--\\
%
%                \hline%==============================================================================================================
%
%                \multicolumn{9}{c}{Fast/Faster-RCNN Re-train}\\
%                \hline
%
%                OM+MIL\hfilll\cite{Li2016}&VGG16&39.5&52.4&--&--\\
%
%                OPG Fast-RCNN\hfilll\cite{Shen2018OPG}&VGG16&31.4&44.5&--&--\\
%
%                OICR Ens. Fast-RCNN\hfilll\cite{Tang2017}&VGG16&47.0&64.3&42.5&65.6\\
%
%                Ge \etal\hfilll\cite{Ge2018}&VGG16&51.2&--&--&--\\
%
%                W2F \etal\hfilll\cite{Zhang}&VGG16&52.4&70.3&47.8&69.4\\
%
%                $TS^2C$\hfilll\cite{Wei2018TS2C}&VGG16&48.0&--&44.4&--\\
%
%                WSRPN Ens.\hfilll\cite{Tang}&VGG16&50.4&68.4&--&--\\
%
%                WSRPN \hfilll\cite{Tang}&VGG16&--&--&45.7&69.3\\
%
%                ML-LocNet\hfilll\cite{Zhang2018g}&VGG16&49.7&--&--&--\\
%                ML-LocNet Ens.\hfilll\cite{Zhang2018g}&VGG16&--&68.6&43.6&68.2\\
%
%                CSC Fast-RCNN\hfilll\cite{Shen2019CSC}&VGG16&49.0&66.1&44.1$^{\S}$&67.0\\
%
%                WS-JDS Fast-RCNN\hfilll\cite{Shen2019WSJDS}&VGG16&52.5&68.6&46.1&69.5\\
%
%                SD-LocNet\hfilll\cite{Zhang2019b}&VGG-M&48.4&67.4&--&--\\
%                SD-LocNet\hfilll\cite{Zhang2019b}&VGG16&51.3&70.9&49.2&69.1&9.7&21.6&--\\
%
%                Kosugi \etal Fast-RCNN\hfilll\cite{Kosugi2019}&VGG16&51.4&--&48.1&--\\
%                Kosugi \etal PGE Fast-RCNN\hfilll\cite{Kosugi2019}&VGG16&52.1&--&47.9&--\\
%
%                C-MIL Fast-RCNN\hfilll\cite{Wan2019}&VGG16&53.1&--&--&--\\
%
%                SDCN Fast-RCNN\hfill \cite{Li2019a}&VGG16&51.0&68.8&46.7&69.5\\
%
%                Sona \emph{et al} Fast-RCNN\hfilll\cite{Sona}&VGG16&48.8&--&--&--\\
%
%                C-MIDN Fast-RCNN\hfilll\cite{CMIDN}&VGG16&53.6&71.9&50.3&73.3\\
%
%                OIM+IR Fast-RCNN\hfilll\cite{Lin2020}&VGG16&52.6&68.8&46.4&69.5\\
%
%                Zeni \etal Fast-RCNN\hfilll\cite{Zeni2020}&VGG16&50.0&--&--&--\\
%
%                PG-PS Faster-RCNN\hfilll\cite{Cheng2020}&VGG16&54.6&72.2&52.9&71.0\\
%
%                \hline%==============================================================================================================

%                \midrule%==============================================================================================================
%                \multicolumn{9}{c}{FSOD}\\
%                \midrule
%
%                Fast RCNN\hfilll\cite{FASTRCNN}&VGG16&66.9&--&65.7&--&18.9&38.6&--\\
%                Faster RCNN\hfilll\cite{FASTERRCNN}&VGG16&69.9&--&67.0&--&21.2&41.5&--\\
%

                \midrule%==============================================================================================================
                \multicolumn{9}{c}{FSOD}\\
                \midrule

                Fast RCNN\hfilll\cite{FASTRCNN}&VGG16&66.9&--&65.7&--&18.9&38.6&--\\
                Faster RCNN\hfilll\cite{FASTERRCNN}&VGG16&69.9&--&67.0&--&21.2&41.5&--\\

%                \midrule%==============================================================================================================
%                \multicolumn{9}{c}{Upper Bound with GT-bbox Known}\\
%                \midrule
%
%                OICR + GAM + REG\hfilll\cite{Yanga}&VGG16&66.9&--&65.7&--&18.9&38.6&--\\
%                Ren \etal\hfilll\cite{Ren2020}&VGG16&66.9&--&65.7&--&18.9&38.6&--\\
%                UWSOD&VGG16&69.9&--&67.0&--&21.2&41.5&--\\

                \midrule%==============================================================================================================
                \multicolumn{9}{c}{WSOD with Cls-agnostic GT-bbox Known}\\
                \midrule

                OICR + GAM + REG\hfilll\cite{Yanga}&VGG16&54.3&81.3&53.9&82.1&13.7&27.1&12.5\\

                Ren \etal\hfilll\cite{Ren2020}&VGG16&62.2&87.1&62.1&88.9&14.1&28.9&12.7\\

                \midrule
                \multirow{2}{*}{UWSOD}&  VGG16  &{67.7}&\textbf{93.3}&{65.3}&91.1&\textbf{15.3}&\textbf{32.4}&\textbf{12.8}\\

                &  WSR18  &\textbf{69.7}&{92.5}&\textbf{66.1}&\textbf{92.3}&{13.7}&{27.9}&{12.5}\\

                \bottomrule%==============================================================================================================

            \end{tabular}
        \end{adjustbox}
    \end{center}
    \label{table_voc2007voc2012mscoco_sota}
%    \vspace{-20pt}
\end{table*}


==> main/table_voc2007voc2012mscoco_wsod_sota.tex <==
\begin{table*}[!h]
%    \vspace{-20pt}
    \caption{
        Comparison with the state-of-the-art methods on PASCAL VOC 2007, 2012 and MS COCO object detection.
%        \scriptsize{
        %    $^{\ddag}$\url{http://host.robots.ox.ac.uk:8080/anonymous/3ESVLJ.html}
        %    $^{\P}$\url{http://host.robots.ox.ac.uk:8080/anonymous/FUTRJO.html}
        %    $^{\$}$\url{http://host.robots.ox.ac.uk:8080/anonymous/ICYSCH.html}
        %    $^{\dag}$\url{http://host.robots.ox.ac.uk:8080/anonymous/WOPMN0.html}
        %    $^{\S}$\url{http://host.robots.ox.ac.uk:8080/anonymous/LX5460.html}
        %    $^{\pounds}$\url{http://host.robots.ox.ac.uk:8080/anonymous/NNFS4F.html}
%        }
    }
    \vspace{-20pt}
    \footnotesize
    \begin{center}
        \begin{adjustbox}{max width=0.9\textwidth}
            \begin{tabular}{l|c|c|cc|cc|ccc}
                \toprule

                \multirow{3}{*}{Method}&\multirow{3}{*}{Supervision}&\multirow{3}{*}{Bakcbone}&\multicolumn{2}{c|}{PASCAL VOC 2007}&\multicolumn{2}{c|}{PASCAL VOC 2012}&\multicolumn{3}{c}{MS COCO}\\

                &&&\multirow{2}{*}{$m$AP (\%)}&\multirow{2}{*}{CorLoc (\%)}&\multirow{2}{*}{$m$AP (\%)}&\multirow{2}{*}{CorLoc (\%)}&\multicolumn{3}{c}{Avg. Precision, IoU:}\\

                &&&&&&&0.5:0.95&0.5&0.75\\
                
                \midrule
                
                Faster RCNN\hfilll\cite{FASTERRCNN}&$\mathcal{B}$&VGG16&69.9&--&67.0&--&21.2&41.5&--\\
                
                
%                \midrule
%                \multicolumn{9}{c}{WSOD {with} external object proposal modules or additional data}\\
                \midrule%==============================================================================================================

%                \multicolumn{9}{c}{Object Discovery}\\
%                \hline

%                Siva \etal\hfilll\cite{siva2012defence}&&--&30.2&--&--&--&--&--\\

%                Shi \etal\hfilll\cite{Shi2017}&&--&36.2&--&--&--&--&--\\

%                Rochan \etal\hfilll\cite{Rochan2015}&AlexNet&--&58.8&--&--&--&--&--\\

%                RMI-SVM\hfilll\cite{Wang2015}&AlexNet&--&40.2&--&--&--&--&--\\

%                STL\hfilll\cite{Bazzani2016}&AlexNet&--&54.4&--&--&--&--&--\\

%                Song \etal\hfilll\cite{Song2014Weakly}&AlexNet&24.6&--&--&--&--&--&--\\

%                Bilen \etal\hfilll\cite{Bilen2014}&AlexNet&26.4&--&--&--&--&--&--\\

%                Cover+SLSVM\hfilll\cite{song2014learning}&AlexNet&22.7&--&--&--&--&--&--\\

%                LCL-pLSA\hfilll\cite{Wang2014}&AlexNet&30.9&48.5&--&--&--&--&--\\
%                LCL+Context\hfilll\cite{Wang2014}&AlexNet&31.6&--&--&--&--&--&--\\

%                Bilen \etal\hfilll\cite{Bilen2015}&AlexNet&27.7&43.7&--&--&--&--&--\\

%                Multi-Fold MIL\hfilll\cite{Cinbis2015}&AlexNet&30.2&52.0&--&--&--&--&--\\

%                Teh\hfilll\cite{Teh2016}&AlexNet&34.5&64.6&--&--&--&--&--\\

%                WSDDN\hfilll\cite{Bilen2016}&VGG-F&34.5&54.2&--&--&--&--&--\\
%                WSDDN\hfilll\cite{Bilen2016}&VGG-M&34.9&56.1&--&--&--&--&--\\
                WSDDN\hfilll\cite{Bilen2016}&$\mathcal{I}$&VGG16&34.8&53.5&--&--&9.5&19.2&8.2\\

%                ContextLocNet\hfilll\cite{Kantorov2016}&VGG-F&36.3&55.1&35.3&54.8&11.1&22.1&10.7\\

%                Beam Search\hfilll\cite{Bency2016}&VGG16&25.7&--&26.5&--&--&--&--\\

%                OM+MIL\hfilll\cite{Li2016}&AlexNet&23.4&41.2&29.1&--&--&--&--\\

%                OPG\hfilll\cite{Shen_2018_TNNLS}&AlexNet&27.0&34.2&--&--&--&--&--\\
                OPG\hfilll\cite{Shen_2018_TNNLS}&$\mathcal{I}$&VGG16&28.8&43.5&--&--&--&--&--\\

%                WCCN\hfilll\cite{Diba2017}&VGG16&42.8&56.7&37.9&--&--&--&--\\

%                Jiang \etal\hfilll\cite{Jiang2017}&AlexNet&37.4&57.3&33.6&--&--&--&--\\

%                Jie \etal\hfilll\cite{Jie2017}&VGG16&41.7&56.1&38.3&58.8&--&--&--\\

%                SPAM-CAM\hfilll\cite{Gudi2017}&VGG16&27.5&--&--&--&--&--&--\\

%                TST\hfilll\cite{Shi2017a}&AlexNet&33.8&59.5&--&--&--&--&--\\

%                SGWSOD\hfilll\cite{Lai2017a}&VGG-F&38.9&60.8&--&--&--&--&--\\
%                SGWSOD\hfilll\cite{Lai2017a}&VGG-M-1024&39.4&59.6&--&--&--&--&--\\
%                SGWSOD\hfilll\cite{Lai2017a}&VGG16&43.5&62.9&39.6&62.9&--&--&--\\

%                TS$^2$C\hfilll\cite{Wei2018TS2C}&VGG16&44.3&61.0&40.0&64.4&--&--&--\\

%                CSC C5\hfilll\cite{Shen_2019_TIP}&VGG-F&38.4&60.4&--&--&--&--&--\\
%                CSC C5\hfilll\cite{Shen_2019_TIP}&VGG-M&39.3&60.6&--&--&--&--&--\\
                CSC C5\hfilll\cite{Shen_2019_TIP}&$\mathcal{I}$&VGG16&43.0&62.2&37.1&61.4&\textbf{12.9}&23.8&\textbf{13.2}\\

                WS-JDS\hfilll\cite{Shen_2019_CVPR}&$\mathcal{I}$&VGG16&45.6&64.5&39.1&63.5&--&--&--\\

%                Oquab \etal\hfilll\cite{Oquab2015}&AlexNet&--&--&11.7&--&--&--&--\\

%                \hline%==============================================================================================================

%                \multirow{4}{*}{WSDDN}\hfilll\multirow{4}{*}{\cite{Bilen2016}}&VGG16&34.8&53.5&--&--\\
%                &ResNet18-WS&43.4&63.1&--&--\\
%                &ResNet50-WS&44.0&63.6&--&--\\
%                &ResNet101-WS&44.1&64.0&--&--\\
%
%                \hline%==============================================================================================================
%
%                \multirow{4}{*}{ContextLocNet}\hfilll\multirow{4}{*}{\cite{Kantorov2016}}&VGG-F&36.3&55.1&35.3&54.8\\
%                &ResNet18-WS&45.4&64.7&42.0$^{\ddag}$&66.7\\
%                &ResNet50-WS&45.3&65.1&--&--\\ %TODO
%                &ResNet101-WS&45.9&65.7&--&--\\ %TODO
%
%                \hline%==============================================================================================================

%                \multicolumn{9}{c}{Object Discovery + Instance Refinement}\\
%                \hline

%                OICR\hfilll\cite{Tang2017}&VGG-M&37.9&57.3&34.6&60.7&--&--&--\\
                OICR\hfilll\cite{Tang2017}&$\mathcal{I}$&VGG16&41.2&60.6&37.9&62.1&--&--&--\\

%                K-EM\hfilll\cite{Yan2017}&VGG16&46.1&65.0&--&--&--&--&--\\

                MELM\hfilll\cite{Wan}&$\mathcal{I}$&VGG16&47.3&61.4&42.4&--&--&--&--\\

%                ZLDN\hfilll\cite{Zhang2018b}&VGG16&47.6&61.2&42.9&61.5&--&--&--\\

%                GAL-fWSD300\hfilll\cite{Shen_2018_CVPR}&VGG16&47.0&68.1&43.1&67.2&--&--&--\\
%                GAL-fWSD512\hfilll\cite{Shen_2018_CVPR}&VGG16&47.5&66.1&--&--&--&--&--\\

%                ML-LocNet\hfilll\cite{Zhang2018g}&VGG-S&44.4&63.7&--&--&--&--&--\\
%                ML-LocNet\hfilll\cite{Zhang2018g}&VGG-M&47.2&65.3&--&--&--&--&--\\
%                ML-LocNet\hfilll\cite{Zhang2018g}&VGG16&48.4&67.0&42.2&66.3&--&16.2&--\\

%                WSRPN\hfilll\cite{Tang}&VGG16&45.3&63.8&40.8&64.9&--&--&--\\

%                PCL\hfilll \cite{Tang2018b}&VGG16&43.5&--&--&--&8.5&19.4&--\\

                Kosugi \etal\hfilll\cite{Kosugi2019}&$\mathcal{I}$&VGG16&47.6&66.7&43.4&66.7&--&--&--\\

%                C-MIL\hfilll\cite{Wan2019}&VGG-F&40.7&--&--&--&--&--&--\\
                C-MIL\hfilll\cite{Wan2019}&$\mathcal{I}$&VGG16&50.5&65.0&46.7&67.4&--&--&--\\

                Pred Net\hfilll\cite{Arun2018a}&$\mathcal{I}$&VGG16&52.9&70.9&48.4&69.5&--&--&--\\

%                WSDDN + W-RPN\hfilll\cite{Singh}&VGG16&39.4&--&--&--&--&--&--\\
%                OICR W-RPN\hfilll\cite{Singh}&VGG16&46.9&--&43.2&67.5&--&--&--\\

%                SDCN\hfilll\cite{Li2019a}&VGG16&48.3&66.8&43.5&67.9&--&--&--\\

%                Sona \etal\hfilll\cite{Sona}&VGG16&45.4&--&--&--&--&--&--\\

                WSOD$^2$\hfilll\cite{Zeng2019}&$\mathcal{I}$&VGG16&53.6&69.5&47.2&{71.9}&10.8&22.7&--\\

                Yanga \etal \hfilll\cite{Yanga}&$\mathcal{I}$&VGG16&48.6&66.8&--&--&--&--&--\\
%                PCL+GAM+REG \hfilll\cite{Yanga}&VGG16&51.5&68.0&--&--&--&--&--\\

                C-MIDN\hfilll\cite{CMIDN}&$\mathcal{I}$&VGG16&52.6&68.7&50.2&71.2&9.6&21.4&--\\

%                OIM\hfilll\cite{Lin2020}&VGG16&48.2&--&--&--&--&--&--\\
%                OIM+IR\hfilll\cite{Lin2020}&VGG16&50.1&67.2&45.3&67.1&--&--&--\\

                Ren \etal\hfilll\cite{Ren2020}&$\mathcal{I}$&VGG16&\textbf{54.9}&68.8&\textbf{52.1}&70.9&12.4&\textbf{25.8}&10.5\\

%                Zeni \etal\hfilll\cite{Zeni2020}&VGG16&49.7&65.7&--&66.3&--&--&--\\

%                PG-PS\hfilll\cite{Cheng2020}&VGG16&51.1&\textbf{69.2}&48.3&68.7&--&20.7&--\\

%                \midrule
%                \multicolumn{9}{c}{WSOD {without} external object proposal modules or additional data}\\
%                \midrule%==============================================================================================================

%                Shi \etal\hfilll\cite{Shi2017}&--&--&36.2&--&--&--&--&--\\

%                Beam Search\hfilll\cite{Bency2016}&VGG16&25.7&--&26.5&--&--&--&--\\

%                OM+MIL\hfilll\cite{Li2016}&AlexNet&23.4&41.2&29.1&--&--&--&--\\

                %OPG\hfilll\cite{Shen_2018_TNNLS}&AlexNet&27.0&34.2&--&--&--&--&--\\
%                OPG\hfilll\cite{Shen_2018_TNNLS}&VGG16&28.8&43.5&--&--&--&--&--\\

%                SPAM-CAM\hfilll\cite{Gudi2017}&VGG16&27.5&--&--&--&--&--&--\\

%                \midrule
%                UWSOD&VGG16&44.0&63.0&45.1&65.2&2.5&9.3&1.1\\
                UWSOD\hfilll~\cite{Shen_2020_NeurIPS}&$\mathcal{I}$&ResNet18-WS&45.0&63.8&46.2&65.7&3.1&10.1&1.4\\

                \midrule
                \multirow{1}{*}{JTSM}&\multirow{1}{*}{$\mathcal{I}$}
                %&VGG16    & 54.9 & 71.9 & 52.5 & 72.0 & 12.8 & 24.0 & 10.9 \\
                %&&ResNet18-WS & 55.3 & 70.6 & \textbf{53.5} & 73.5 & 13.0 & 25.0 & 11.4 \\
                &ResNet18-WS & 53.4 & \textbf{71.4} & 51.5 & \textbf{72.5} & 9.4 & 21.3 & 7.9 \\
                %&&ResNet50-WS & 55.8 & 71.1 & 53.4 & \textbf{73.7} & \textbf{13.3} & 25.2 & 11.2 \\
                %&&ResNet101-WS& \textbf{55.9} & \textbf{71.3} & 53.2 & 73.6 & 13.1 & 25.3 & \textbf{11.6} \\

%                \midrule%==============================================================================================================
%
%                \multirow{4}{*}{OICR}\hfilll\multirow{4}{*}{\cite{Tang2017}}&VGG16&41.2&60.6&37.9&62.1\\
%                &ResNet18-WS&51.0&68.7&&\\
%                &ResNet50-WS&50.9&67.4&50.4$^{\P}$&72.5\\
%                &ResNet101-WS&51.4&68.9&48.6$^{\$}$&70.3\\
%
%                \hline%==============================================================================================================
%
%                \multirow{4}{*}{PCL}\hfilll\multirow{4}{*}{\cite{Tang2018b}}&VGG16&43.5&62.7&40.6&63.2\\
%                &ResNet18-WS&50.2&67.1&--&--\\
%                &ResNet18-WS F2&51.9&70.1&--&--\\
%                &ResNet50-WS&50.8&67.8&--&--\\
%                &ResNet101-WS&54.3&72.0&51.2$^{\dag}$&73.5\\
%
%                \hline%==============================================================================================================
%
%                \multirow{4}{*}{C-MIL}\hfilll\multirow{4}{*}{\cite{Wan2019}}&VGG16&50.5&65.0&46.7&67.4\\
%                &ResNet18-WS&52.6&68.5&50.6$^{\S}$&73.0\\
%                &ResNet50-WS&53.4&69.3&--&--\\ %TODO
%                &ResNet101-WS&55.9&72.4&--&--\\ %TODO
%
%                \hline%==============================================================================================================
%
%                \multirow{2}{*}{OICR+GAM+REG}\hfilll\multirow{2}{*}{\cite{Yanga}}&VGG16&48.6&66.8&46.8&69.5\\
%                &ResNet101-WS&59.5&81.3&59.1$^{\pounds}$&81.0\\
%
%                \hline%==============================================================================================================
%
%                \multicolumn{9}{c}{Ensemble}\\
%                \hline
%                WSDDN Ens.\hfilll\cite{Bilen2016}&&39.3&58.0&--&--\\
%
%                OICR Ens.\hfilll\cite{Tang2017}&&42.0&61.2&38.2&63.5\\
%
%                SGWSOD Ens.\hfilll\cite{Lai2017a}&&43.9&63.6&40.6&64.2\\
%
%                Ge \etal Ens.\hfilll\cite{Ge}&&43.9&58.3&--&--\\
%
%                CSC Ens.\hfilll\cite{Shen_2019_TIP}&&43.5&63.7&--&--\\
%
%                WSRPN Ens.\hfilll\cite{Tang}&&47.9&66.9&43.4&67.2\\
%
%                Pred Net Ens.\hfilll\cite{Arun2018a}&&53.6&71.4&49.5&70.2\\
%
%                MIL+GAM+REG-Ens. \hfilll\cite{Yanga}&&54.5&--&--&--\\
%
%                \hline%==============================================================================================================
%
%                \multicolumn{9}{c}{Fast/Faster-RCNN Re-train}\\
%                \hline
%
%                OM+MIL\hfilll\cite{Li2016}&VGG16&39.5&52.4&--&--\\
%
%                OPG Fast-RCNN\hfilll\cite{Shen_2018_TNNLS}&VGG16&31.4&44.5&--&--\\
%
%                OICR Ens. Fast-RCNN\hfilll\cite{Tang2017}&VGG16&47.0&64.3&42.5&65.6\\
%
%                Ge \etal\hfilll\cite{Ge2018}&VGG16&51.2&--&--&--\\
%
%                W2F \etal\hfilll\cite{Zhang}&VGG16&52.4&70.3&47.8&69.4\\
%
%                $TS^2C$\hfilll\cite{Wei2018TS2C}&VGG16&48.0&--&44.4&--\\
%
%                WSRPN Ens.\hfilll\cite{Tang}&VGG16&50.4&68.4&--&--\\
%
%                WSRPN \hfilll\cite{Tang}&VGG16&--&--&45.7&69.3\\
%
%                ML-LocNet\hfilll\cite{Zhang2018g}&VGG16&49.7&--&--&--\\
%                ML-LocNet Ens.\hfilll\cite{Zhang2018g}&VGG16&--&68.6&43.6&68.2\\
%
%                CSC Fast-RCNN\hfilll\cite{Shen_2019_TIP}&VGG16&49.0&66.1&44.1$^{\S}$&67.0\\
%
%                WS-JDS Fast-RCNN\hfilll\cite{Shen_2019_CVPR}&VGG16&52.5&68.6&46.1&69.5\\
%
%                SD-LocNet\hfilll\cite{Zhang2019b}&VGG-M&48.4&67.4&--&--\\
%                SD-LocNet\hfilll\cite{Zhang2019b}&VGG16&51.3&70.9&49.2&69.1&9.7&21.6&--\\
%
%                Kosugi \etal Fast-RCNN\hfilll\cite{Kosugi2019}&VGG16&51.4&--&48.1&--\\
%                Kosugi \etal PGE Fast-RCNN\hfilll\cite{Kosugi2019}&VGG16&52.1&--&47.9&--\\
%
%                C-MIL Fast-RCNN\hfilll\cite{Wan2019}&VGG16&53.1&--&--&--\\
%
%                SDCN Fast-RCNN\hfill \cite{Li2019a}&VGG16&51.0&68.8&46.7&69.5\\
%
%                Sona \emph{et al} Fast-RCNN\hfilll\cite{Sona}&VGG16&48.8&--&--&--\\
%
%                C-MIDN Fast-RCNN\hfilll\cite{CMIDN}&VGG16&53.6&71.9&50.3&73.3\\
%
%                OIM+IR Fast-RCNN\hfilll\cite{Lin2020}&VGG16&52.6&68.8&46.4&69.5\\
%
%                Zeni \etal Fast-RCNN\hfilll\cite{Zeni2020}&VGG16&50.0&--&--&--\\
%
%                PG-PS Faster-RCNN\hfilll\cite{Cheng2020}&VGG16&54.6&72.2&52.9&71.0\\
%
%                \hline%==============================================================================================================

%                \midrule%==============================================================================================================
%                \multicolumn{9}{c}{FSOD}\\
%                \midrule
%
%                Fast RCNN\hfilll\cite{FASTRCNN}&VGG16&66.9&--&65.7&--&18.9&38.6&--\\
%                Faster RCNN\hfilll\cite{FASTERRCNN}&VGG16&69.9&--&67.0&--&21.2&41.5&--\\
%

%                \midrule%==============================================================================================================
%                \multicolumn{9}{c}{FSOD}\\
%                \midrule

%                Fast RCNN\hfilll\cite{FASTRCNN}&VGG16&66.9&--&65.7&--&18.9&38.6&--\\
%                Faster RCNN\hfilll\cite{FASTERRCNN}&VGG16&69.9&--&67.0&--&21.2&41.5&--\\

%                \midrule%==============================================================================================================
%                \multicolumn{9}{c}{Upper Bound with GT-bbox Known}\\
%                \midrule
%
%                OICR + GAM + REG\hfilll\cite{Yanga}&VGG16&66.9&--&65.7&--&18.9&38.6&--\\
%                Ren \etal\hfilll\cite{Ren2020}&VGG16&66.9&--&65.7&--&18.9&38.6&--\\
%                UWSOD&VGG16&69.9&--&67.0&--&21.2&41.5&--\\


                \bottomrule%==============================================================================================================
            \end{tabular}
        \end{adjustbox}
    \end{center}
    \label{table_voc2007voc2012mscoco_wsod_sota}
    \vspace{-20pt}
\end{table*}


==> main/table_voc2010voc2012_sota.tex <==

\begin{table}[t]
    \begin{minipage}[t]{.5\linewidth}
        %\vspace{-15pt}
        \caption{
            %Comparison with the state-of-the-art methods on PASCAL VOC 2012 in terms of mAP (\%) and CorLoc (\%).
            Comparison with the state-of-the-art methods on VOC 2012 in terms of mAP and CorLoc.
            %
            %\scriptsize{
            %    $^{\ddag}$\url{http://host.robots.ox.ac.uk:8080/anonymous/4LLJNW.html}
            %    $^{\P}$\url{http://host.robots.ox.ac.uk:8080/anonymous/FUTRJO.html}
            %    $^{\$}$\url{http://host.robots.ox.ac.uk:8080/anonymous/ICYSCH.html}
            %    $^{\dag}$\url{http://host.robots.ox.ac.uk:8080/anonymous/WOPMN0.html}
            %    $^{\S}$\url{http://host.robots.ox.ac.uk:8080/anonymous/LX5460.html}
            %    $^{\pounds}$\url{http://host.robots.ox.ac.uk:8080/anonymous/NNFS4F.html}
            %}
        }
        \vspace{-5pt}
        \footnotesize
        \begin{center}
            \begin{adjustbox}{max width=1.0\textwidth}
                \begin{tabular}{l|cc}
                    \hline
                    Method&$m$AP (\%)&CorLoc (\%)\\
                    
                    \hline
                    \multicolumn{3}{c}{Object Mining}\\
                    %==============================================================================================================
                    \hline
                    
                    %Oquab \etal\hfilll\cite{Oquab2015} &11.7&--\\
                    
                    %Multi-Fold MIL\hfilll\cite{Cinbis2015}     &27.4&55.2&--&--\\
                    
                    ContextLocNet\hfilll\cite{Kantorov2016}    &35.3&54.8\\
                    
                    %Beam Search\hfilll\cite{Bency2016}         &26.5&--\\
                    
                    %OM + MIL\hfilll\cite{Li2016}               &29.1&--\\
                    
                    %WCCN\hfilll\cite{Diba2017}                 &37.9&--\\
                    
                    Jie \etal\hfilll\cite{Jie2017}              &38.3&58.8\\
                    
                    SGWSOD\hfilll\cite{Lai2017a}               &39.6&62.9\\
                    
                    TS$^2$C\hfilll\cite{Wei2018TS2C}           &40.0&64.4\\
                    
                    %CSC\hfilll\cite{Shen_2019_TIP}             &37.6$^{\ddag}$&61.0&37.1$^{\dag}$&61.4\\
                    %CSC\hfilll\cite{Shen_2019_TIP}             &37.1$^{\dag}$&61.4\\
                    
                    %WS-JDS\hfilll\cite{Shen_2019_CVPR}         &{39.9}&{63.1}&{39.1}&63.5\\
                    %WS-JDS\hfilll\cite{Shen_2019_CVPR}         &{39.1}&63.5\\
                    
                    
                    %==============================================================================================================
                    %\hline
                    %\multirow{4}{*}{WSDDN}\hfilll\multirow{4}{*}{\cite{Bilen2016}}
                    %&ResNet18-WS&\\
                    %&ResNet50-WS&\\
                    %&ResNet101-WS&&\\
                    
                    %==============================================================================================================
                    %\hline
                    %\multirow{5}{*}{ContextLocNet}\hfilll\multirow{5}{*}{\cite{Kantorov2016}}
                    %&35.3&54.8\\
                    %&ResNet18-WS&42.0$^{\ddag}$&66.7\\ %TODO
                    %&ResNet50-WS&\\
                    %&ResNet101-WS&&\\
                    
                    %==============================================================================================================
                    \hline
                    \multicolumn{3}{c}{Object Mining + Instance Refinement}\\
                    \hline
                    
                    %OICR\hfilll\cite{Tang2017}                     &34.6&60.7\\
                    OICR\hfilll\cite{Tang2017}                     &37.9&62.1\\
                    
                    MELM\hfilll\cite{Wan}                          &42.4&--\\
                    
                    ZLDN\hfilll\cite{Zhang2018b}                   &42.9&61.5\\
                    
                    WSRPN\hfilll\cite{Tang}                        &40.8&64.9\\
                    
                    %GAL-fWSD300\hfilll\cite{Shen_2018_CVPR}        &45.1&68.3&43.1&67.2\\
                    %GAL-fWSD300\hfilll\cite{Shen_2018_CVPR}        &43.1&67.2\\
                    
                    Kosugi \etal\hfilll\cite{Kosugi2019}           &43.4&66.7\\
                    
                    ML-LocNet\hfilll\cite{Zhang2018g}              &42.2&66.3\\
                    
                    C-MIL\hfilll\cite{Wan2019}               &46.7&67.4\\
                    
                    Pred Net\hfilll\cite{Arun2018a}          &48.4&69.5\\
                    
                    OICR + W-RPN\hfilll\cite{Singh}                &43.2&67.5\\
                    
                    SDCN\hfilll\cite{Li2019a}                      &43.5&67.9\\
                    
                    WSOD$^2$\hfilll\cite{Zeng2019}                 &47.2&71.9\\
                    
                    OIM+IR\hfilll\cite{Lin2020}                    &45.3&67.1\\
                    
                    C-MIDN\hfilll\cite{CMIDN}                      &50.2&71.2\\
                    
                    Ren \etal\hfilll\cite{Ren2020}                 &52.1&70.9\\
                    
                    BOICR\hfilll\cite{Zeni2020}                    &--&66.3\\
                    
                    PG-PS\hfilll\cite{Cheng2020}                   &48.3&68.7\\
                    
                    %==============================================================================================================
                    \hline
                    UWSOD&&\\
                    
                    
                    %==============================================================================================================
                    \hline
                    \multicolumn{3}{c}{FSOD}\\
                    \hline
                    
                    Fast RCNN\hfilll\cite{FASTRCNN}&65.7&--\\
                    
                    Faster RCNN\hfilll\cite{FASTERRCNN}&67.0&--\\
                    
                    %==============================================================================================================
                    %\hline
                    %\multirow{6}{*}{OICR}\hfilll\multirow{6}{*}{\cite{Tang2017}}
                    %&37.9&62.1\\
                    %&ResNet18-WS&\\
                    %&ResNet50-WS&\\
                    %&ResNet101-WS&50.4$^{\P}$&72.5\\
                    %&DenseNet121-WS&48.6$^{\$}$&70.3\\ %TODO
                    
                    %==============================================================================================================
                    %\hline
                    %\multirow{5}{*}{PCL}\hfilll\multirow{5}{*}{\cite{Tang2018b}}
                    %&40.6&63.2\\
                    %&ResNet18-WS&\\
                    %&ResNet50-WS&\\
                    %&ResNet101-WS&51.2$^{\dag}$&73.5\\
                    
                    %==============================================================================================================
                    %\hline
                    %\multirow{5}{*}{C-MIL}\hfilll\multirow{5}{*}{\cite{Wan2019}}
                    %&46.7&67.4\\
                    %&ResNet18-WS&50.6$^{\S}$&73.0\\
                    %&ResNet50-WS&\\
                    %&ResNet101-WS&&\\
                    
                    %==============================================================================================================
                    %\hline
                    %\multirow{5}{*}{OICR+GAM+REG}\hfilll\multirow{5}{*}{\cite{Yanga}}
                    %&46.8&69.5\\
                    %&ResNet18-WS&\\
                    %&ResNet50-WS&\\
                    %&ResNet101-WS&59.1$^{\pounds}$&81.0\\ %TODO
                    
                    %==============================================================================================================
                    %\hline
                    %\multicolumn{4}{c}{Ensemble}\\
                    %\hline
                    
                    %OICR Ens.\hfilll\cite{Tang2017}            &&38.2&63.5\\
                    
                    %SGWSOD VGG16\hfilll\cite{Lai2017a}         &&40.6&64.2\\
                    
                    %WSRPN Ens.\hfilll\cite{Tang}  &&43.4&67.2\\
                    
                    %Pred Net Ens.\hfilll\cite{Arun2018a}       &&49.5&70.2\\
                    
                    %==============================================================================================================
                    %\hline
                    %\multicolumn{4}{c}{Fast/Faster-RCNN Re-train}\\
                    %\hline
                    
                    %OICR Ens.\hfilll\cite{Tang2017}                 &42.5&65.6\\
                    
                    %W2F\hfilll\cite{Zhang}                           &{47.8}&{69.4}\\
                    
                    %TS$^2$C\hfilll\cite{Wei2018TS2C}                 &44.4&--\\
                    
                    %WSRPN\hfilll\cite{Tang}                          &45.7&69.3\\
                    
                    %CSC Fast-RCNN\hfilll\cite{Shen_2019_TIP}                   &43.7$^{\P}$&66.2&44.1$^{\S}$&67.0\\
                    %CSC Fast-RCNN\hfilll\cite{Shen_2019_TIP}                   &44.1$^{\S}$&67.0\\
                    
                    %WS-JDS Fast-RCNN\hfilll\cite{Shen_2019_CVPR}               &{45.7}&{68.1}&46.1&{69.5}\\
                    %WS-JDS Fast-RCNN\hfilll\cite{Shen_2019_CVPR}               &46.1&{69.5}\\
                    
                    %SD-LocNet\hfilll\cite{Zhang2019b}                              &49.2&69.1\\
                    
                    %Kosugi \etal Fast-RCNN\hfilll\cite{Kosugi2019}        &48.1&--\\
                    %Kosugi \etal PGE Fast-RCNN\hfilll\cite{Kosugi2019}    &47.9&--\\
                    
                    %ML-LocNet Ens.\hfilll\cite{Zhang2018g}                         &43.6&68.2\\
                    
                    %SDCN Fast-RCNN\hfill \cite{Li2019a}                            &46.7&69.5\\
                    
                    %C-MIDN FRCNN\hfilll\cite{CMIDN}                        &50.3&73.3\\
                    
                    %OIM+IR FRCNN\hfilll\cite{Lin2020}                      &46.4&69.5\\
                    
                    %PG-PS FRCNN\hfilll\cite{Cheng2020}                     &52.9&71.0\\
                    
                    %==============================================================================================================
                    \hline
                \end{tabular}
            \end{adjustbox}
        \end{center}
        \label{table_voc2010voc2012_sota}
        \vspace{-20pt}
    \end{minipage} 

    \begin{minipage}[t]{.5\linewidth}
        \centering
        %\vspace{-15pt}
        \caption{Comparisons with the state-of-the-art methods on COCO minival set.}
        \vspace{-5pt}
        \footnotesize
        \begin{center}
            \begin{adjustbox}{max width=1.0\linewidth}
                \centering
                %\vspace{-5.0pt}
                %\begin{tabular}{l|c|ccc|ccc|ccc|ccc}
                %\begin{tabular}{l|c|ccc|ccc}
                \begin{tabular}{l|ccc}
                    \hline
                    %\multirow{2}{*}{Method} & \multirow{2}{*}{Bakcbone} & \multicolumn{3}{c|}{\scriptsize{Avg. Precision, IoU:}} & \multicolumn{3}{c}{\scriptsize{Avg. Precision, Area:}}& \multicolumn{3}{c|}{\scriptsize{Avg. Recall, \#Dets:}} & \multicolumn{3}{c}{\scriptsize{Avg. Recall, Area:}}\\
                    %\multirow{2}{*}{Method} & \multirow{2}{*}{Bakcbone} & \multicolumn{3}{c|}{\scriptsize{Avg. Precision, IoU:}} & \multicolumn{3}{c}{\scriptsize{Avg. Precision, Area:}}\\
                    \multirow{2}{*}{Method} & \multicolumn{3}{c}{\scriptsize{Avg. Precision, IoU:}} \\
                    
                    %& & 0.5:0.95 & 0.5 & 0.75 & S & M & L & 1 & 10 & 100 & S & M & L\\
                    %& & 0.5:0.95 & 0.5 & 0.75 & S & M & L \\
                    & 0.5:0.95 & 0.5 & 0.75 \\
                    %==============================================================================================================
                    \hline
                    
                    % wsddn_vgg16_coco_2019-07-03_01-19-17
                    %WSDDN$^*$                                                          &10.2&20.4&08.8&02.2&11.0&18.9&13.0&24.8&26.9&05.7&29.6&50.2\\
                    WSDDN$^*$                                                          &10.2&20.4&08.8\\
                    
                    % wsddn_vgg_cnn_m_coco_2019-07-31_02-58-46
                    %WSDDN$^*$                                                          &08.8&17.1&07.9&01.3&08.4&15.9&11.7&21.9&23.6&04.1&23.6&46.2\\
                    
                    % wsddn_vgg_cnn_f_coco_2019-07-30_17-30-43
                    %WSDDN$^*$                                                          & VGG-F &08.6&16.5&07.8&01.6&08.8&15.3&11.4&21.7&23.3&04.0&23.7&45.7\\
                    
                    % csc_vgg16_coco_2019-07-05_01-54-02
                    %CSC C5                                                             &10.2&20.3&08.9&02.3&10.9&18.5&13.0&24.8&26.7&05.2&28.6&50.2\\
                    
                    % paper
                    %WSDDN \hfilll\cite{Bilen2016}                                      &9.5&19.2&8.2&2.1&10.4&17.2&12.2&23.6&25.3&6.3&25.7&48.2\\
                    WSDDN \hfilll\cite{Bilen2016}                                      &9.5&19.2&8.2\\
                    
                    % paper
                    %ContextLocNet\hfilll\cite{Kantorov2016}                            &11.1&22.1&10.7&{2.9}&12.4&19.2&{12.2}&{24.5}&24.3&{6.5}&28.7&49.3\\
                    ContextLocNet\hfilll\cite{Kantorov2016}                            &11.1&22.1&10.7\\
                    
                    % paper
                    %CSC C5\hfilll\cite{Shen_2019_TIP}                                  &{12.9}&{23.8}&{13.2}&{2.9}&{12.5}&{20.3}&{12.2}&23.9&{25.7}&6.1&{29.7}&{49.7}\\
                    
                    %Diba \etal\hfilll\cite{Diba2017a}        & VGG16 (14train/14test) &--&12.8&--&--&--&--\\
                    Diba \etal\hfilll\cite{Diba2017a}        &--&12.8&---\\
                    
                    %SD-LocNet\hfilll\cite{Zhang2019b}        & VGG16 (14train/14val)&9.7&21.6&--&--&--&--\\
                    SD-LocNet\hfilll\cite{Zhang2019b}        &9.7&21.6&---\\
                    
                    %ML-LocNet\hfilll\cite{Zhang2018g}        & VGG-S (14train/14val) &--&16.2&--&--&--&--\\
                    ML-LocNet\hfilll\cite{Zhang2018g}        &--&16.2&--\\
                    
                    %WSOD$^2$\hfilll\cite{Zeng2019}          & VGG16 (14train/14val)&10.8&22.7&--&--&--&--\\
                    WSOD$^2$\hfilll\cite{Zeng2019}          &10.8&22.7&--\\
                    
                    %PCL\hfilll\cite{Tang2018b}&VGG-M(14train/14val)&7.3&16.6&--&--&--&--\\
                    %PCL\hfilll\cite{Tang2018b}&VGG16(14train/14val)&8.5&19.4&--&--&--&--\\
                    PCL\hfilll\cite{Tang2018b}&8.5&19.4&--\\
                    %PCL Fast RCNN\hfilll\cite{Tang2018b}&VGG16(14train/14val)&9.2&19.6&--&--&--&--\\
                    
                    %C-MIDN\hfilll\cite{CMIDN}&VGG16(14train/14val)&9.6&21.4&--&--&--&--\\
                    C-MIDN\hfilll\cite{CMIDN}&9.6&21.4&--\\
                    
                    %PG-PS\hfilll\cite{Cheng2020}&VGG16(14train/14val)&--&20.7&--&--&--&--\\
                    PG-PS\hfilll\cite{Cheng2020}&--&20.7&--\\
                    
                    %PML-LocNet-S\hfilll\cite{Zhang2020a}&VGG16(14train/14val)&--&21.6&--&--&--&--\\
                    %PML-LocNet-L\hfilll\cite{Zhang2020a}&VGG16(14train/14val)&--&20.9&--&--&--&--\\
                    PML-LocNet-L\hfilll\cite{Zhang2020a}&--&20.9&--\\
                    
                    %==============================================================================================================
                    %\hline
                    
                    %\multirow{4}{*}{WSDDN}\hfilll\multirow{4}{*}{\cite{Bilen2016}}&9.5&19.2&8.2&2.1&10.4&17.2\\
                    %&12.2&23.6&25.3&6.3&25.7&48.2\\
                    %&ResNet18-WS&11.3&22.0&10.0&2.7&11.9&21.4\\
                    %&ResNet50-WS&\\ %TODO
                    %&ResNet101-WS&\\ %TODO
                    
                    %==============================================================================================================
                    %\hline
                    
                    %\multirow{4}{*}{ContextNet}\hfilll\multirow{4}{*}{\cite{Kantorov2016}}&11.1&22.1&10.7&{2.9}&12.4&19.2\\
                    %&{12.2}&{24.5}&24.3&{6.5}&28.7&49.3\\
                    %&ResNet18-WS&15.0&25.9&13.8&4.2&15.1&24.4\\ %TODO
                    %&ResNet50-WS&\\ %TODO
                    %&ResNet101-WS&\\ %TODO
                    
                    %==============================================================================================================
                    \hline
                    
                    \multirow{3}{*}{Ren \etal}\hfilll\multirow{3}{*}{\cite{Ren2020}} 
                    %&VGG16(14train/14val)&11.4&24.3&9.4&8.5&25.4&38.3\\
                    &11.4&24.3&9.4\\
                    %&R50-C4 (14train/14val)&12.6&26.1&10.8&8.4&25.1&41.8\\
                    %&R50-C4 &12.6&26.1&10.8\\
                    %&R101-C4 (14train/14val)&13.0&26.3&11.4&8.5&24.6&40.9\\
                    %&R101-C4 &13.0&26.3&11.4\\
                    %&VGG16(17train/minival)&12.4&25.8&10.5&9.7&26.6&39.6\\
                    &12.4&25.8&10.5\\
                    %&VGG16(14train/Test-Dev)&12.1&24.8&10.2&9.6&30.0&46.7\\
                    &12.1&24.8&10.2\\
                    
                    %==============================================================================================================
                    \hline
                    UWSOD&&&\\
                    
                    %==============================================================================================================
                    \hline
                    \multicolumn{4}{c}{FSOD}\\
                    \hline
                    
                    Fast RCNN\hfilll\cite{FASTRCNN}&18.9&38.6&--\\
                    
                    Faster RCNN\hfilll\cite{FASTERRCNN}&21.2&41.5&--\\
                    
                    %Faster RCNN\hfilll\cite{FASTERRCNN}&R101&27.2&48.4&--\\
                    
                    %==============================================================================================================
                    \hline
                \end{tabular}
                %\vspace{-5.0pt}
            \end{adjustbox}
        \end{center}
        \vspace{-20pt}
        \label{table_coco_sota_map}
    \end{minipage} 
\end{table}


==> main/table_voc2010voc2012_sota_net.tex <==
\begin{table}[t]
    \begin{minipage}[t]{.5\linewidth}
    %\vspace{-15pt}
    \caption{
        %Comparison with the state-of-the-art methods on PASCAL VOC 2012 in terms of mAP (\%) and CorLoc (\%).
        Comparison with the state-of-the-art methods on VOC 2012 in terms of mAP and CorLoc.
        %
        %\scriptsize{
        %    $^{\ddag}$\url{http://host.robots.ox.ac.uk:8080/anonymous/4LLJNW.html}
        %    $^{\P}$\url{http://host.robots.ox.ac.uk:8080/anonymous/FUTRJO.html}
        %    $^{\$}$\url{http://host.robots.ox.ac.uk:8080/anonymous/ICYSCH.html}
        %    $^{\dag}$\url{http://host.robots.ox.ac.uk:8080/anonymous/WOPMN0.html}
        %    $^{\S}$\url{http://host.robots.ox.ac.uk:8080/anonymous/LX5460.html}
        %    $^{\pounds}$\url{http://host.robots.ox.ac.uk:8080/anonymous/NNFS4F.html}
        %}
    }
    \vspace{-5pt}
    \footnotesize
    \begin{center}
        \begin{adjustbox}{max width=1.0\textwidth}
            \begin{tabular}{l|l|cc}
                \hline
                Method&Backbone&$m$AP (\%)&CorLoc (\%)\\
                
                \hline
                \multicolumn{4}{c}{Object Mining}\\
                %==============================================================================================================
                \hline
                
                %Oquab \etal\hfilll\cite{Oquab2015} &AlexNet&11.7&--\\
                
                %Multi-Fold MIL\hfilll\cite{Cinbis2015}     &AlexNet&27.4&55.2&--&--\\
                
                ContextLocNet\hfilll\cite{Kantorov2016}    &VGG-F&35.3&54.8\\
                
                %Beam Search\hfilll\cite{Bency2016}         &VGG16&26.5&--\\
                
                %OM + MIL\hfilll\cite{Li2016}               &AlexNet&29.1&--\\
                
                %WCCN\hfilll\cite{Diba2017}                 &VGG16&37.9&--\\
                
                Jie \etal\hfilll\cite{Jie2017}              &VGG16&38.3&58.8\\
                
                SGWSOD\hfilll\cite{Lai2017a}               &VGG16&39.6&62.9\\
                
                TS$^2$C\hfilll\cite{Wei2018TS2C}           &VGG16&40.0&64.4\\
                
                %CSC\hfilll\cite{Shen_2019_TIP}             &VGG16&37.6$^{\ddag}$&61.0&37.1$^{\dag}$&61.4\\
                %CSC\hfilll\cite{Shen_2019_TIP}             &VGG16&37.1$^{\dag}$&61.4\\
                
                %WS-JDS\hfilll\cite{Shen_2019_CVPR}         &VGG16&{39.9}&{63.1}&{39.1}&63.5\\
                %WS-JDS\hfilll\cite{Shen_2019_CVPR}         &VGG16&{39.1}&63.5\\
                
                
                %==============================================================================================================
                %\hline
                %\multirow{4}{*}{WSDDN}\hfilll\multirow{4}{*}{\cite{Bilen2016}}
                %&ResNet18-WS&\\
                %&ResNet50-WS&\\
                %&ResNet101-WS&&\\
                
                %==============================================================================================================
                %\hline
                %\multirow{5}{*}{ContextLocNet}\hfilll\multirow{5}{*}{\cite{Kantorov2016}}
                %&VGG-F&35.3&54.8\\
                %&ResNet18-WS&42.0$^{\ddag}$&66.7\\ %TODO
                %&ResNet50-WS&\\
                %&ResNet101-WS&&\\
                
                %==============================================================================================================
                \hline
                \multicolumn{4}{c}{Object Mining + Instance Refinement}\\
                \hline
                
                %OICR\hfilll\cite{Tang2017}                     &VGG-M&34.6&60.7\\
                OICR\hfilll\cite{Tang2017}                     &VGG16&37.9&62.1\\
                
                MELM\hfilll\cite{Wan}                          &VGG16&42.4&--\\
                
                ZLDN\hfilll\cite{Zhang2018b}                   &VGG16&42.9&61.5\\
                
                WSRPN\hfilll\cite{Tang}                        &VGG16&40.8&64.9\\
                
                %GAL-fWSD300\hfilll\cite{Shen_2018_CVPR}        &VGG16&45.1&68.3&43.1&67.2\\
                %GAL-fWSD300\hfilll\cite{Shen_2018_CVPR}        &VGG16&43.1&67.2\\
                
                Kosugi \etal\hfilll\cite{Kosugi2019}           &VGG16&43.4&66.7\\
                
                ML-LocNet\hfilll\cite{Zhang2018g}              &VGG16&42.2&66.3\\
                
                C-MIL\hfilll\cite{Wan2019}               &VGG16&46.7&67.4\\
                
                Pred Net\hfilll\cite{Arun2018a}          &VGG16&48.4&69.5\\
                
                OICR + W-RPN\hfilll\cite{Singh}                &VGG16&43.2&67.5\\
                
                SDCN\hfilll\cite{Li2019a}                      &VGG16&43.5&67.9\\
                
                WSOD$^2$\hfilll\cite{Zeng2019}                 &VGG16&47.2&71.9\\
                
                OIM+IR\hfilll\cite{Lin2020}                    &VGG16&45.3&67.1\\
                
                C-MIDN\hfilll\cite{CMIDN}                      &VGG16&50.2&71.2\\
                
                Ren \etal\hfilll\cite{Ren2020}                 &VGG16&52.1&70.9\\
                
                BOICR\hfilll\cite{Zeni2020}                    &VGG16&--&66.3\\
                
                PG-PS\hfilll\cite{Cheng2020}                   &VGG16&48.3&68.7\\
                
                %==============================================================================================================
                \hline
                UWSOD&VGG16&&\\
                
                
                %==============================================================================================================
                \hline
                \multicolumn{4}{c}{FSOD}\\
                \hline
                
                Fast RCNN\hfilll\cite{FASTRCNN}&VGG16&65.7&--\\
                
                Faster RCNN\hfilll\cite{FASTERRCNN}&VGG16&67.0&--\\
                
                %==============================================================================================================
                %\hline
                %\multirow{6}{*}{OICR}\hfilll\multirow{6}{*}{\cite{Tang2017}}
                %&VGG16&37.9&62.1\\
                %&ResNet18-WS&\\
                %&ResNet50-WS&\\
                %&ResNet101-WS&50.4$^{\P}$&72.5\\
                %&DenseNet121-WS&48.6$^{\$}$&70.3\\ %TODO
                
                %==============================================================================================================
                %\hline
                %\multirow{5}{*}{PCL}\hfilll\multirow{5}{*}{\cite{Tang2018b}}
                %&VGG16&40.6&63.2\\
                %&ResNet18-WS&\\
                %&ResNet50-WS&\\
                %&ResNet101-WS&51.2$^{\dag}$&73.5\\
                
                %==============================================================================================================
                %\hline
                %\multirow{5}{*}{C-MIL}\hfilll\multirow{5}{*}{\cite{Wan2019}}
                %&VGG16&46.7&67.4\\
                %&ResNet18-WS&50.6$^{\S}$&73.0\\
                %&ResNet50-WS&\\
                %&ResNet101-WS&&\\
                
                %==============================================================================================================
                %\hline
                %\multirow{5}{*}{OICR+GAM+REG}\hfilll\multirow{5}{*}{\cite{Yanga}}
                %&VGG16&46.8&69.5\\
                %&ResNet18-WS&\\
                %&ResNet50-WS&\\
                %&ResNet101-WS&59.1$^{\pounds}$&81.0\\ %TODO
                
                %==============================================================================================================
                %\hline
                %\multicolumn{4}{c}{Ensemble}\\
                %\hline
                
                %OICR Ens.\hfilll\cite{Tang2017}            &&38.2&63.5\\
                
                %SGWSOD VGG16\hfilll\cite{Lai2017a}         &&40.6&64.2\\
                
                %WSRPN Ens.\hfilll\cite{Tang}  &&43.4&67.2\\
                
                %Pred Net Ens.\hfilll\cite{Arun2018a}       &&49.5&70.2\\
                
                %==============================================================================================================
                %\hline
                %\multicolumn{4}{c}{Fast/Faster-RCNN Re-train}\\
                %\hline
                
                %OICR Ens.\hfilll\cite{Tang2017}                 &VGG16&42.5&65.6\\
                
                %W2F\hfilll\cite{Zhang}                           &VGG16&{47.8}&{69.4}\\
                
                %TS$^2$C\hfilll\cite{Wei2018TS2C}                 &VGG16&44.4&--\\
                
                %WSRPN\hfilll\cite{Tang}                          &VGG16&45.7&69.3\\
                
                %CSC Fast-RCNN\hfilll\cite{Shen_2019_TIP}                   &VGG16&43.7$^{\P}$&66.2&44.1$^{\S}$&67.0\\
                %CSC Fast-RCNN\hfilll\cite{Shen_2019_TIP}                   &VGG16&44.1$^{\S}$&67.0\\
                
                %WS-JDS Fast-RCNN\hfilll\cite{Shen_2019_CVPR}               &VGG16&{45.7}&{68.1}&46.1&{69.5}\\
                %WS-JDS Fast-RCNN\hfilll\cite{Shen_2019_CVPR}               &VGG16&46.1&{69.5}\\
                
                %SD-LocNet\hfilll\cite{Zhang2019b}                              &VGG16&49.2&69.1\\
                
                %Kosugi \etal Fast-RCNN\hfilll\cite{Kosugi2019}        &VGG16&48.1&--\\
                %Kosugi \etal PGE Fast-RCNN\hfilll\cite{Kosugi2019}    &VGG16&47.9&--\\
                
                %ML-LocNet Ens.\hfilll\cite{Zhang2018g}                         &VGG16&43.6&68.2\\
                
                %SDCN Fast-RCNN\hfill \cite{Li2019a}                            &VGG16&46.7&69.5\\
                
                %C-MIDN FRCNN\hfilll\cite{CMIDN}                        &VGG16&50.3&73.3\\
                
                %OIM+IR FRCNN\hfilll\cite{Lin2020}                      &VGG16&46.4&69.5\\
                
                %PG-PS FRCNN\hfilll\cite{Cheng2020}                     &VGG16&52.9&71.0\\
                
                %==============================================================================================================
                \hline
            \end{tabular}
        \end{adjustbox}
    \end{center}
    \label{table_voc2010voc2012_sota}
    \vspace{-20pt}
    
\end{minipage} 
    \begin{minipage}[t]{.5\linewidth}
        \centering
        %\vspace{-15pt}
        \caption{Comparisons with the state-of-the-art methods on COCO minival set.}
        \vspace{-5pt}
        \footnotesize
        \begin{center}
            \begin{adjustbox}{max width=1.0\linewidth}
                \centering
                %\vspace{-5.0pt}
                %\begin{tabular}{l|c|ccc|ccc|ccc|ccc}
                %\begin{tabular}{l|c|ccc|ccc}
                \begin{tabular}{l|c|ccc}
                    \hline
                    %\multirow{2}{*}{Method} & \multirow{2}{*}{Bakcbone} & \multicolumn{3}{c|}{\scriptsize{Avg. Precision, IoU:}} & \multicolumn{3}{c}{\scriptsize{Avg. Precision, Area:}}& \multicolumn{3}{c|}{\scriptsize{Avg. Recall, \#Dets:}} & \multicolumn{3}{c}{\scriptsize{Avg. Recall, Area:}}\\
                    %\multirow{2}{*}{Method} & \multirow{2}{*}{Bakcbone} & \multicolumn{3}{c|}{\scriptsize{Avg. Precision, IoU:}} & \multicolumn{3}{c}{\scriptsize{Avg. Precision, Area:}}\\
                    \multirow{2}{*}{Method} & \multirow{2}{*}{Bakcbone} & \multicolumn{3}{c}{\scriptsize{Avg. Precision, IoU:}} \\
                    
                    %& & 0.5:0.95 & 0.5 & 0.75 & S & M & L & 1 & 10 & 100 & S & M & L\\
                    %& & 0.5:0.95 & 0.5 & 0.75 & S & M & L \\
                    & & 0.5:0.95 & 0.5 & 0.75 \\
                    %==============================================================================================================
                    \hline
                    
                    % wsddn_vgg16_coco_2019-07-03_01-19-17
                    %WSDDN$^*$                                                          &VGG16&10.2&20.4&08.8&02.2&11.0&18.9&13.0&24.8&26.9&05.7&29.6&50.2\\
                    WSDDN$^*$                                                          &VGG16&10.2&20.4&08.8\\
                    
                    % wsddn_vgg_cnn_m_coco_2019-07-31_02-58-46
                    %WSDDN$^*$                                                          &VGG-M&08.8&17.1&07.9&01.3&08.4&15.9&11.7&21.9&23.6&04.1&23.6&46.2\\
                    
                    % wsddn_vgg_cnn_f_coco_2019-07-30_17-30-43
                    %WSDDN$^*$                                                          &VGG-F&08.6&16.5&07.8&01.6&08.8&15.3&11.4&21.7&23.3&04.0&23.7&45.7\\
                    
                    % csc_vgg16_coco_2019-07-05_01-54-02
                    %CSC C5                                                             &VGG16&10.2&20.3&08.9&02.3&10.9&18.5&13.0&24.8&26.7&05.2&28.6&50.2\\
                    
                    % paper
                    %WSDDN \hfilll\cite{Bilen2016}                                      &VGG16&9.5&19.2&8.2&2.1&10.4&17.2&12.2&23.6&25.3&6.3&25.7&48.2\\
                    WSDDN \hfilll\cite{Bilen2016}                                      &VGG16&9.5&19.2&8.2\\
                    
                    % paper
                    %ContextLocNet\hfilll\cite{Kantorov2016}                            &VGG16&11.1&22.1&10.7&{2.9}&12.4&19.2&{12.2}&{24.5}&24.3&{6.5}&28.7&49.3\\
                    ContextLocNet\hfilll\cite{Kantorov2016}                            &VGG16&11.1&22.1&10.7\\
                    
                    % paper
                    %CSC C5\hfilll\cite{Shen_2019_TIP}                                  &VGG16&{12.9}&{23.8}&{13.2}&{2.9}&{12.5}&{20.3}&{12.2}&23.9&{25.7}&6.1&{29.7}&{49.7}\\
                    
                    %Diba \etal\hfilll\cite{Diba2017a}        &VGG-F(14train/14test) &--&12.8&--&--&--&--\\
                    Diba \etal\hfilll\cite{Diba2017a}        &VGG16&--&12.8&---\\
                    
                    %SD-LocNet\hfilll\cite{Zhang2019b}        &VGG-F(14train/14val)&9.7&21.6&--&--&--&--\\
                    SD-LocNet\hfilll\cite{Zhang2019b}        &VGG16&9.7&21.6&---\\
                    
                    %ML-LocNet\hfilll\cite{Zhang2018g}        &VGG-S(14train/14val) &--&16.2&--&--&--&--\\
                    ML-LocNet\hfilll\cite{Zhang2018g}        &VGG-S&--&16.2&--\\
                    
                    %WSOD$^2$\hfilll\cite{Zeng2019}          &VGG-F(14train/14val)&10.8&22.7&--&--&--&--\\
                    WSOD$^2$\hfilll\cite{Zeng2019}          &VGG16&10.8&22.7&--\\
                    
                    %PCL\hfilll\cite{Tang2018b}&VGG-M(14train/14val)&7.3&16.6&--&--&--&--\\
                    %PCL\hfilll\cite{Tang2018b}&VGG16(14train/14val)&8.5&19.4&--&--&--&--\\
                    PCL\hfilll\cite{Tang2018b}&VGG16&8.5&19.4&--\\
                    %PCL Fast RCNN\hfilll\cite{Tang2018b}&VGG16(14train/14val)&9.2&19.6&--&--&--&--\\
                    
                    %C-MIDN\hfilll\cite{CMIDN}&VGG16(14train/14val)&9.6&21.4&--&--&--&--\\
                    C-MIDN\hfilll\cite{CMIDN}&VGG16&9.6&21.4&--\\
                    
                    %PG-PS\hfilll\cite{Cheng2020}&VGG16(14train/14val)&--&20.7&--&--&--&--\\
                    PG-PS\hfilll\cite{Cheng2020}&VGG16&--&20.7&--\\
                    
                    %PML-LocNet-S\hfilll\cite{Zhang2020a}&VGG16(14train/14val)&--&21.6&--&--&--&--\\
                    %PML-LocNet-L\hfilll\cite{Zhang2020a}&VGG16(14train/14val)&--&20.9&--&--&--&--\\
                    PML-LocNet-L\hfilll\cite{Zhang2020a}&VGG16&--&20.9&--\\
                    
                    %==============================================================================================================
                    %\hline
                    
                    %\multirow{4}{*}{WSDDN}\hfilll\multirow{4}{*}{\cite{Bilen2016}}&VGG16&9.5&19.2&8.2&2.1&10.4&17.2\\
                    %&12.2&23.6&25.3&6.3&25.7&48.2\\
                    %&ResNet18-WS&11.3&22.0&10.0&2.7&11.9&21.4\\
                    %&ResNet50-WS&\\ %TODO
                    %&ResNet101-WS&\\ %TODO
                    
                    %==============================================================================================================
                    %\hline
                    
                    %\multirow{4}{*}{ContextNet}\hfilll\multirow{4}{*}{\cite{Kantorov2016}}&VGG16&11.1&22.1&10.7&{2.9}&12.4&19.2\\
                    %&{12.2}&{24.5}&24.3&{6.5}&28.7&49.3\\
                    %&ResNet18-WS&15.0&25.9&13.8&4.2&15.1&24.4\\ %TODO
                    %&ResNet50-WS&\\ %TODO
                    %&ResNet101-WS&\\ %TODO
                    
                    %==============================================================================================================
                    \hline
                    
                    \multirow{5}{*}{Ren \etal}\hfilll\multirow{5}{*}{\cite{Ren2020}} 
                    %&VGG16(14train/14val)&11.4&24.3&9.4&8.5&25.4&38.3\\
                    &VGG16&11.4&24.3&9.4\\
                    %&R50-C4(14train/14val)&12.6&26.1&10.8&8.4&25.1&41.8\\
                    &R50-C4&12.6&26.1&10.8\\
                    %&R101-C4(14train/14val)&13.0&26.3&11.4&8.5&24.6&40.9\\
                    &R101-C4&13.0&26.3&11.4\\
                    %&VGG16(17train/minival)&12.4&25.8&10.5&9.7&26.6&39.6\\
                    &VGG16&12.4&25.8&10.5\\
                    %&VGG16(14train/Test-Dev)&12.1&24.8&10.2&9.6&30.0&46.7\\
                    &VGG16&12.1&24.8&10.2\\
                    
                    %==============================================================================================================
                    \hline
                    UWSOD&VGG16&&&\\
                    
                    %==============================================================================================================
                    \hline
                    \multicolumn{4}{c}{FSOD}\\
                    \hline
                    
                    Fast RCNN\hfilll\cite{FASTRCNN}&VGG16&18.9&38.6&--\\
                    
                    Faster RCNN\hfilll\cite{FASTERRCNN}&VGG16&21.2&41.5&--\\
                    
                    Faster RCNN\hfilll\cite{FASTERRCNN}&R101&27.2&48.4&--\\
                    
                    %==============================================================================================================
                    \hline
                \end{tabular}
                %\vspace{-5.0pt}
            \end{adjustbox}
        \end{center}
        \vspace{-20pt}
        \label{table_coco_sota_map}
    \end{minipage} 
\end{table}

